SoK: Plausibly Deniable Storage

Data privacy is critical in instilling trust and empowering the societal pacts of modern technology-driven democracies. Unfortunately, it is under continuous attack by overreaching or outright oppressive governments, including some of the world's oldest democracies. Increasingly-intrusive anti-encryption laws severely limit the ability of standard encryption to protect privacy. New defense mechanisms are needed. Plausible deniability (PD) is a powerful property, enabling users to hide the existence of sensitive information in a system under direct inspection by adversaries. Popular encrypted storage systems such as TrueCrypt and other research efforts have attempted to also provide plausible deniability. Unfortunately, these efforts have often operated under less well-defined assumptions and adversarial models. Careful analyses often uncover not only high overheads but also outright security compromise. Further, our understanding of adversaries, the underlying storage technologies, as well as the available plausible deniable solutions have evolved dramatically in the past two decades. The main goal of this work is to systematize this knowledge. It aims to: - identify key PD properties, requirements, and approaches; - present a direly-needed unified framework for evaluating security and performance; - explore the challenges arising from the critical interplay between PD and modern system layered stacks; - propose a new "trace-oriented" PD paradigm, able to decouple security guarantees from the underlying systems and thus ensure a higher level of flexibility and security independent of the technology stack. This work is meant also as a trusted guide for system and security practitioners around the major challenges in understanding, designing, and implementing plausible deniability into new or existing systems.

==> conclusion.tex <==
%!TEX root=../main.tex

\section{Conclusion}

Plausible deniability can provide strong privacy guarantees that impacts millions of users in a world increasingly encroaching on encryption and personal privacy. Yet, building secure plausibly deniable efficient systems is far from trivial. This work systematizes existing knowledge for researchers and practitioners alike aiming to understand, deploy, or design plausible deniability systems. We believe plausible deniability to be an important property on the cusp of efficient mainstream practicality. This work is meant as a concise yet reasonably-complete guide on this journey.


==> hide_access_pattern.tex <==
%!TEX root=main.tex

\section{Hiding Access Patterns}
\label{section:hide-hidden-access}

\subsection{Single-Snapshot Adversaries}

To achieve single-snapshot security, existing works explore two major directions. 

The first direction is inspired by classical {\em steganography}, i.e., embedding relatively small messages within large cover-texts, such as adding imperceptible echoes at certain places in an audio recording \cite{petitcolas1999information}. Anderson \etal \cite{anderson1998steganographic} explored steganographic file systems and proposed two approaches for hiding data.
The first approach defines the target file as the (password-derived) linear combination of a set of cover files. 
The second approach encrypts the target file using a block cipher with password-derived secret keys, and then stores it at the location determined by a cryptographic hash of the filename. In both approaches, an adversary without the correct password can get no information about whether the protected file ever exists. The latter approach was later implemented and optimized by McDonald \etal \cite{mcdonald1999stegfs} and Pang \etal \cite{pang2003stegfs}. Unfortunately, such approaches are not extremely space-effective, and come with potential data loss and high performance overheads. They are not suited for building modern systems handling large amounts of data at high speed.

The second direction \cite{Truecrypt,skillen2013mobiflage,jia2017deftl} handles PD at block-device level by designing disk encryption tools that help users embed ``hidden volumes'' (together with ``public volumes'') within the device (e.g., in the free space regions), while preventing adversaries from learning how many such volumes the device actually contains. Different keys are used to encrypt different volumes using randomized encryption indistinguishable from pseudo-random free space noise. Upon coercion, a user can provide the encryption keys for the public volumes, thus providing a plausible non-hidden use case for the disk. The adversary does not have any evidence for the existence of additional volumes.

{\bf TrueCrypt} \cite{Truecrypt} successfully implemented this idea. It stores hidden volumes in the free space of public volumes. To hide their existence, TrueCrypt fills all free space with random data and encrypts the hidden data with a semantically secure encryption scheme that has pseudo-random ciphertexts. Upon coercion, the user can reveal the keys for the public volumes, and claim that the remaining space contains random free space. Rubberhose \cite{rubberhose}, MobiFlage \cite{skillen2013implementing} and DEFTL \cite{jia2017deftl} are implementations following  similar ideas targeted to different use cases (mobile devices, NAND flash). 

\subsection{Single vs. Multi-snapshot Adversary}

While single-snapshot security is easy to achieve with low overheads and high performance, it does not protect against realistic adversaries who are often more powerful and can gain access to the device more than once during their life time (``multi-snapshot'' adversary).

And unfortunately, all the aforementioned schemes fail to protect against multi-snapshot adversaries. As a simple powerful example consider that when TrueCrypt writes hidden data, the device ``free space'' changes unexplainably. When observed by a multi-snapshot adversary this cannot be plausibly explained away. After all, why did the disk free area change without corresponding substantial changes to the public data?

This seems to suggest that, to protect against multi-snapshot adversaries, one needs to {\em hide not only the existence of hidden data, but also associated access patterns.}

\begin{mybox}{}
The essence of multi-snapshot resilient PD systems lies in hiding the access patterns to hidden data.
\end{mybox}

Given this insight, progress in this area centers mainly around mechanisms that can consistently explain updates to both the public and hidden data across multiple snapshots. Currently, three major approaches exist: (i) using oblivious RAM mechanisms (ORAMs), (ii) using canonical forms and (iii) relying on device/deployment-specific properties. The remainder of this section will explore these approaches, aiming to understand the fundamentals and distill insights to guide future designs. 

\subsection{ORAM-Based PD Schemes}
\label{sec:hide_pattern_ORAM}

Multi-snapshot secure PD requires mechanisms that hide users' access patterns to hidden data. ORAMs \cite{goldreich1996software} are natural tools for this task. 

\noindent{\em ORAMs.} Roughly, an ORAM ensures a database-hosting server cannot determined which database (the ``RAM'') entries are accessed by one of its client. Access patterns of any same-length access sequences are designed to be indistinguishable. As a simple example, a (highly inefficient yet secure) ORAM (with $O(n)$ asymptotic complexity per access) can be constructed by filling the database with randomized encrypted data; To access one of the elements, the client reads the entire database, re-encrypts it and writes it back to the server. More efficient solutions exist that enable complexities much lower than $O(n)$ \cite{stefanov2011towards,stefanov2013path,DBLP:conf/ndss/ChakrabortiACMR19,DBLP:conf/ndss/ChakrabortiS19,DBLP:journals/popets/ChakrabortiS20}.  An exhaustive treatment is out of scope here. The following summarizes how ORAMs were employed to obtain PD solutions. 

\subpara{HIVE \cite{blass2014toward}} was the first to deploy ORAMs. It introduced ``hidden volume encryption''. The main idea was similar to a previous work \cite{Truecrypt}---it basically divides the storage into a public volume and a hidden volume\footnote{The original HIVE scheme supports multiple volumes. W.l.o.g., only the two-volume case is considered here (for simplicity).}, each volume being accessed using an ORAM mechanism. 
%
Additionally, for every access to a volume (either public or hidden), the system also executes ``dummy'' accesses to the other volume. Since ORAM accesses are indistinguishable from each other (whether ``dummy'' or not), adversaries cannot tell the difference between 1) accesses to the public volume and 2) accesses to the hidden volume, {\em which satisfies the exact requirement of the CPA game for PD}.

Moreover, the authors observe that  \Read operations are not visible to adversaries since such operations do not leave any discernible traces. Thus, it is sufficient to use write-only ORAM schemes (see \Cref{def:wORAM}) that only hide \Write operations. HIVE designed a specific write-only ORAM with a stash.

Finally, it is observed in \cite{blass2014toward} that the write-only ORAM stash can also behave as a queue for caching hidden data, and hidden volume accesses can be performed together with existing (if any) public volume accesses to minimize the need for additional ``dummy''. In this case, the adversary cannot tell the difference between 1) accesses to the public volume only and 2) accesses to both public and hidden volumes. The only associated requirement now becomes the need for enough plausible public accesses to pair with the hidden data in the stash when written to disk. 

\subpara{DataLair \cite{chakraborti2017datalair}} extends these ideas and observes that operations on public data do not need to be hidden since they are anyway public. In fact, revealing operations on public data reinforces deniability as it
shows plausible non-hidden device use. Therefore, DataLair only uses $\wORAM$s for the hidden volumes, while allowing public data to be accessed (almost) directly without any oblivious access mechanism. Moreover, it designs a specific throughput-optimized \wORAM. Following the strategy of HIVE, it pairs the operations on hidden data with those on public data, and ensures that such executions are indistinguishable from the operations on public data alone. Compared with its predecessors, DataLair accelerates public operations by two orders of magnitude, and also speeds up hidden operations.

\para{Where to Write.} An important factor affecting both the security and efficiency of ORAM-based PD approaches \cite{blass2014toward,chakraborti2017datalair} is {\em free-block allocation} (FBA), i.e.~the mechanism to keep track of free blocks to store new incoming data. 

Note that HIVE uses separate ORAMs on public and hidden storage spaces, and DataLair uses ORAM only for hidden space. A naive approach would be to have separate FBA mechanisms for public and hidden spaces.
Unfortunately, this can lead to storage capacity waste, as the hidden space must be allocated even if it is never used. Instead, a better solution uses a ``global'' FBA algorithm across all the storage space. In this case, both the public and the hidden volume can be of the same logical size as the underlying partition, and use all the available space for either hidden or public data.

However, this turns to be a delicate task due to the existence of hidden data. On the one hand, the FBA should avoid overwriting existing hidden data; On the other hand, such avoidance should be strategically hidden to not raise doubts from the adversary about the existence of hidden data.

Moreover, since it is in the data path, FBA must be efficient. Significant amount of work has been devoted \cite{blass2014toward,chakraborti2017datalair} to the design of FBA algorithms that meet the above criteria. The reader is referred to the original papers for details. 

\begin{mybox}{}
ORAMs are powerful tools that can be used in building PD schemes with strong security guarantees. But ORAM-based solutions are inefficient due to the inherently heavy randomization machinery. ORAMs require carefully-designed free-block allocation algorithms.
\end{mybox}

\subsection{Replacing Randomization with Canonical Forms}
\label{section:canonical-forms}

ORAMs are used in PD designs because they can hide both the locations and contents of each access, mostly via inherently high-overhead randomization. 

Yet, randomization is not really necessary to achieve plausible deniability\cite{chen2019}. Simple canonical forms -- e.g., such as used in log-structured file systems \cite{douglis1989log} always writing data sequentially, treating the logical address space as a circular buffer -- may be enough to decouple the user's logical from physical access patterns.

Since canonical forms ensure pre-defined physical device write traces, an adversary is prevented from inferring the logical layer access patterns, of which the traces are independent of. 

Further, importantly, an advantage of certain canonical forms (e.g., sequential) is the ability to retain data locality and thus result in significantly higher efficiency than randomization-based ORAM approaches. 


\subpara{PD-DM \cite{chen2019}} is the first work that {\em explicitly} notes the above idea. Its design ensures that all writes to the physical device are located at sequentially increasing physical addresses, similar to \texttt{Append} operations in log-structure file systems. PD-DM stipulates that whenever a public data record $D_\pub$ is written on the device, an additional random string $R$ (the ``payload'') is written immediately in the immediately adjacent next block. To store hidden data, PD-DM will first encrypt it (indistinguishably from random) and then write it as  the payload of some public data write $D_\pub$. In this case, device snapshots look like the following:

\begin{center}
\vspace{-7pt}
\begin{tikzpicture}[
long/.style = {rectangle, 
                  thin,
                  %draw=black, 
                  fill=white, 
                  align=center,
                  minimum height=15pt,
                  minimum width=30pt},
large/.style = {rectangle, 
                  thin,
                  %draw=black, 
                  fill=white, 
                  align=center,
                  minimum height=15pt,
                  minimum width=26pt},
small/.style = {rectangle, 
                  thin,
                  %draw=black, 
                  fill=white, 
                  align=center,
                  minimum height=15pt,
                  minimum width=15pt},
]
\node [large] (l1) {$D_\pub$};
\draw [thick] (l1.south west) -- (l1.north west);
\draw [densely dashed] (l1.south east) -- (l1.north east);
\node [small, right = 0pt of l1] (s1) {$R$};

\node [large, right = 0pt of s1] (l2) {$D_\pub$};
\draw [thick] (l2.south west) -- (l2.north west);
\draw [densely dashed] (l2.south east) -- (l2.north east);
\node [small, right = 0pt of l2] (s2) {$R$};

\node [long, right = 0pt of s2] (long) {$\cdots$};
\draw [thick] (long.south west) -- (long.north west);

\node [large, right = 0pt of long] (l3) {$D_\pub$};
\draw [thick] (l3.south west) -- (l3.north west);
\draw [densely dashed] (l3.south east) -- (l3.north east);
\node [small, right = 0pt of l3] (s3) {$R$};

\node [long, right = 0pt of s3] (long2) {$\cdots$};
\draw [thick] (long2.south west) -- (long2.north west);

\draw [thick] (l1.north west) -- (long2.north east);
\draw [thick] (l1.south west) -- (long2.south east);
\end{tikzpicture}
\vspace{-10pt}
\end{center}

Since the encrypted hidden data looks indistinguishable from the random ``payload'' of public writings, adversaries are unable to distinguish whether any hidden data exists or not. 

\subpara{ECD \cite{zuck2017preserving}} implicitly work in a related manner. The idea is to partition the device into a public and a hidden volume. The public volume is managed by the system in the standard way, independent of the hidden one. The hidden volume is divided into equal-size sequential {\em segments}, denoted as $\Set{s_1 , s_2, \ldots, s_N}$. Each $s_i$ contains some free blocks containing random strings, while other blocks may be occupied by encrypted hidden data. ECD keeps moving data from $s_{i-1}$ to $s_i$ at a predetermined rate. During this procedure, any free blocks will be re-randomized, while existing hidden data blocks will be re-encrypted. To a polynomial adversary this looks like all of $s_i$ is re-randomized. New hidden data is written encrypted into a free block during the migration from $s_{i-1}$ to $s_i$. Overall this can be viewed as creating an artificial canonical form on the hidden volume, where segment $s_i$ is periodically overwritten by its immediate predecessor $s_{i-1}$. 

\begin{mybox}{}
When used in place of ORAMs to hide user access patterns, canonical forms can result in significant throughput increases. Sequential approaches work particularly well since they can preserve data locality and make good use of locality-optimized systems deploying caching and read-ahead mechanisms. 
\end{mybox}

\subsection{Device-Specific Mechanisms}
\label{sec:fine-tuned-solution}
In pursuit of performance, a recent line of work emerged building plausible deniability guarantees on device-specific properties such as electric charge levels in flash memories etc. This enjoys certain advantages over previous work: 1) it may avoid heavy machinery (e.g., ORAMs) and may lead to lightweight solutions; 2) resulting mechanisms may be closer or even native to the underlying device, allowing for higher performance and better plausibility. 

This approach was often implicit in the literature. This section seeks to sublimate the essence of such constructions in a unified perspective. First, consider several existing constructions. 

\subpara{INFUSE \cite{chen2020infuse}} builds a PD scheme in the flash \FTL layer. The main idea is to modulate additional information in charges and voltage levels of individual NAND cells, the minimal storage unit for NAND. A cell can hold one (SLC, single-level cell) or more (MLC, multiple-level cell) data bits. Bits are encoded and decoded by using a programmable {\em threshold voltage} $V_{\mathsf{th}}$ and a predefined {\em reference voltage} $V_{\mathsf{r}}$. For example, an SLC cell with threshold voltage $V_{\mathsf{th}} = 3V$ will be interpreted as a logical ``1'' when the reference voltage level is $V_{\mathsf{r}} = 3.5V$, and as a ``0'' if either (i) the reference voltage level drops below $V_{\mathsf{r}} = 2.5V$ or (ii) the threshold voltage is increased to e.g., $V_{\mathsf{th}} = 4V$. MLC work similarly, with multiple levels to encode multiple values. 

Some recent flash controllers are able to operate the same cell in both SLC and MLC mode \cite{lee2009flexfs}. This provides an opportunity to hide bits. Multiple bits can be stored in a particular cell using an ``MLC-style'' encoding but on inspection the system can claim that the cell is in SLC mode and provide only a single bit. Care needs to be taken to ensure device-wide indistinguishability between sets of cells in either SLC or MLC mode. This constitutes the core idea of INFUSE. 

Under the (mostly empirical) assumption that an adversary cannot distinguish which cells are used in which mode or whether there are any inconsistencies in the distribution of SLC vs MLC cells, this scheme provides significant speedups. Public data operations are orders of magnitude faster than existing multi-snapshot resilient PD systems, and only 15\% slower than a standard non-PD baseline and hidden data operations perform comparably to the-state-of-the-art PD systems.

\subpara{PEARL \cite{chen2020pearl}} is also operating in the \FTL layer, but relies on a new smart {\em write-once memory} (WOM) encoding that does not require custom voltage programming. 

Unfortunately, once written to, a NAND flash cell cannot be reprogrammed before an ERASE of its containing block. And NAND flash reliably works only for a limited number of ERASE cycles. This can severely limit device lifespan. Complex wear leveling algorithms are deployed to ``even out'' wear and maximize lifespan. 

WOM codes \cite{rivest1982reuse} have been proposed to further optimize this wear. They use an important property of NAND flash: previously-unwritten-to cells can be written to even if they are in pages that have been written to before. 
WOM codes encode with enough redundancy (e.g.~using 3 cells to store 2 bits) to allow {\em multiple} writes to the same page (i.e., with different data each time) without requiring an ERASE. 

At a high level, in the subsequent (e.g., second) \Write, the idea is to modify only the bits that have not been written-to in the first \Write. If the encoding is carefully designed this allows the second logical \Write to be encoded in the resulting physical state with no ambiguity. 

For example, consider the case of an encoding with 2-bit logical data records encoded onto 3 physical bits. For each 2-bit logical record $s\in \bits^2$ the encoding defines two possible physical 3-bit configurations $\Enc_1(s)$ and $\Enc_2(s)$.  When logical record $s$ is stored {\em for the first time}, $\Enc_1(s)$ is stored physically. If the logical record $s$ needs to be replaced with a new value $s'$ (at the same location) writing simply converts the physical value $\Enc_1(s)$ to $\Enc_2(s')$. The WOM encoding is designed unambiguously and in such a way that any such conversion does not require overwriting an existing written-to cell. Since such a code allows two \Write operations per erasure, it is called a 2-write WOM code\footnote{W.l.o.g., for simplicity this work focuses on 2-write WOM codes. But note that there exist $k$-write WOM codes that admit $k$ writings per erasure~\cite{godlewski1987wom,yaakobi2012codes,shpilka2013new}. }.

PEARL \cite{chen2020pearl} hides information by {\em modulating the written public data according to the data to be hidden}. To this end, it re-purposes WOM codes. When public data is written the codeword is chosen based on the bits of the data that needs to be hidden. This enables PEARL to sureptitiously hide information even in the presence of a powerful multi-snapshot adversary. The end-result is device state that is indistinguishable from the case of a device that was simply writing data multiple times using a WOM code. Much care needs to be taken in the design of the specific WOM code to not introduce device-wide bias etc. Overall however, the fact that WOM codes are widely deployed on NAND flash further strengthens plausibility. Most importantly, the resulting performance is comparable to the non-PD baseline on real-world workloads!

\subpara{DEFY \cite{DBLP:conf/ndss/PetersGP15}} is a log-structured \FS for NAND flash that offers PD with a newly proposed secure deletion technology. It is based on WhisperYAFFS~\cite{whisper}, a log structured \FS which provides full disk encryption for flash.  Log-structured {\FS}es have two relevant properties:

\begin{enumerate}
\item
Data (files, directories, links, etc.) and metadata are stored sequentially within the logical address space, and any access to data (including \Read) can cause the update of its corresponding metadata;
\item
Updates/deletes of data and metadata will not cause an actual deletion. Instead, a new address will be assigned to the updated version, and the old data/metadata is just marked as old; Subsequent garbage collection handles it.
\end{enumerate} 

DEFY achieves PD by exploiting the above properties in the following way. In DEFY, modifications to hidden data will cause the allocation of new records. Such allocations can be claimed as the results of metadata updating due to public \Read/\Write, since such updating can also lead to the assignment of new records. Once these records (for hidden data) become obsolete (i.e.~succeeded by newly allocated records), the system can claim that they were due to pubic accesses and are now securely deleted. Due to the irreversibility of secure deletion, the adversary has no choice but to believe that these records were due to public accesses. The system thus denies the existence of hidden data successfully.

DEFY enjoys impressive efficiency. \Read operation can be as fast as the Linux EXT4 file system. 

Unfortunately DEFY is not secure. A related attack shows how DEFY can be easily compromised in a few attempts to exhaust the writing capacity \cite{jia2017deftl}. 

Also, as hidden data are stored masqueraded as securely deleted obsolete (public) data, to maintain plausibility, the space occupied by them must be plausibly and frequently enough overwritten by public data. This results in data loss. Finally, DEFY needs to securely hide a small ``tag storage area'' from adversaries which breaks security against multi-snapshot adversaries. These problems undermine DEFY's practicality and security, despite its appealing efficiency.

\para{In summary}, these schemes are optimized for specific deployment cases. INFUSE and PEARL exploit voltage variation and properties of WOM codes respectively, to encode hidden data together with public data at the same locations. DEFY plausibly encodes hidden data as securely-deleted obsolete public data. The resulting solutions are specific to the underlying devices but achieve performance comparable to the non-PD baseline on real-world workloads. Such efficiency is clearly out of the reach of ORAM-based solutions. Importantly WOM code based schemes provide an unusually favorable combination of strong security and high performance.

\begin{mybox}{}
By exploiting specific devices and deployment settings, lightweight PD systems can be designed, with efficiency comparable to the non-PD baselines. This does not always need to come at the expense of strong security. 
\end{mybox}

\subsection{Access Pattern Hiding Techniques}
\label{sec:ana_access_pattern}

As mentioned earlier, the essence of PD schemes is to conceal access patterns to hidden data. In order to hide the existence of hidden data, a PD scheme should prevent adversaries from learning not only {\it which hidden access happens}, but also {\it how many hidden accesses happen}.
This is in contrast to ORAMs where only that the access patterns of logical requests are not revealed, while the number of accesses can be public.

To hide {\em which hidden access happens}, existing PD schemes leverage one of the following two strategies: 1) randomizing the write trace on physical devices; 2) enforcing the write trace to follow certain canonical form (the commonly used one is log-structure).
Specifically, HIVE, DataLair and MobiCeal \cite{chang2018mobiceal} follow the first strategy; PD-DM, ECD, DEFY, INFUSE and PEARL follow the second strategy. The last 3 schemes are designed for NAND flash devices, where the device is written sequentially by default. To hide the number of hidden accesses, the first strategy is to make the change of device state due to a hidden access to be indistinguishable from that of some non-hidden accesses. Thus, any changes on the devices can be attributed to certain public accesses, and the number of hidden accesses can be claimed as 0. 
Note that the public accesses used to ``explain'' hidden accesses do not need to happen in reality. 
The PD schemes that use this strategy are HIVE, DEFY, PEARL and ECD. 
The first 3 schemes explain a hidden access as either a public \Read, $\mathtt{Delete}$ or \Write, while ECD explains a hidden access as a system behavior that happens at a pre-defined rate. 
Another strategy to hide the number of hidden accesses is to ``pair'' hidden accesses with some public accesses and ensure that write trace of the public accesses alone is indistinguishable from that of both the public accesses and hidden accesses. As a result,
for an adversary, only public accesses happen. Examples include HIVE-B, DataLair, PD-DM, Mobiceal and INFUSE.

\begin{mybox}{}
To design a new PD scheme against multi-snapshot adversary, one can either come up with a new strategy to hide the number of hidden accesses, or a new strategy to hide which hidden access happens, and then combine it with some of the exiting strategies listed above. Finding new strategies for hiding the number of hidden accesses seems more promising as there could be different ways to interpret the disk changes resulting from hidden accesses.
\end{mybox}

\subsection{Invisible PD}

Typically, PD systems only intend to hide the existence of hidden data, not the fact that {\it the system in use is PD}. One can argue that the deployment of a PD system already raises suspicion about the existence of sensitive data.\footnote{Similar debates also exist for deniable encryption \cite{canetti1997deniable,DBLP:conf/crypto/CanettiPP20}.}

To equip the user with more credibility in face of coercive authorities, it is desirable to have {\it invisible} PD schemes that hide not only contents but also the evidence that the system is being used to hide data. This can be done by, e.g., making the scheme look indistinguishable to a off-the-shelf storage system. For instance, StegFS \cite{mcdonald2000steganographic} was designed to be indistinguishable to EXT2. However, StegFS \cite{mcdonald2000steganographic} needs to also maintain a bitmap. Future efforts may look into making this scheme fully indistinguishable by removing the bitmap, while not compromising security.

Further, INFUSE \cite{chen2020infuse} was designed to indistinguishable from YAFFS \cite{yaffs}. There are however two obstacles that prevent it from being practical. First, it has a limited capacity for hidden data: If too much hidden data is stored, the distribution of cell voltages may become suspicious. Second, this scheme requires the firmware support which allows precise manipulation on flash cell voltages. However, current NAND flash chips do not have the corresponding interface admitting such manipulations. Partial programming are used to achieve approximate results.



==> layer_dependence.tex <==
%!TEX root=main.tex

\section{Dependence on Storage Layers}
\label{section:depedence-on-layers}

The layered structure of modern storage systems (details in \Cref{section:storage-layer-prelim}) complicates the design of PD schemes. Consider the ubiquitous modern typical stack: file system (\FS), FS caches, LVM layers, LVM caches, block-devices (\BD), block device caches, and flash translation layers (\FTL), etc. Such a stack includes tens of additional layers and information sources that a single-layer design simply cannot take into account. 

Yet, this is often overlooked and has not been studied in a systematic way. This section will investigate carefully how the security of PD solutions get affected by storage layers. Most importantly, a new ``trace-oriented'' definition for PD will be presented. In a standard PD definition, the adversary gets to see snapshots of devices; A trace-oriented notion allows the adversary to learn operation traces. i.e., the ordered sequence of operations the system performs on the underlying device, independent of layers or device properties\footnote{This should be reminiscent of the requirement for ORAMs}. Trace-oriented PD provides stronger security guarantees and more flexible deployment choices due to its reduced dependence on storage layers. Trace-oriented PD is as powerful as write-only ORAMs and already achieved by several existing constructions.

\subsection{Existing Solutions are Layer-Specific }
\label{sec:layer-dependency}

Because of the layered nature of modern technology stacks, PD solutions end up being designed for a target layer $\Lay$, e.g., $\Lay$ could be $\FS$, $\BD$, $\FTL$ etc. Then, in the security analysis, even the very existence of the underlying layers is often simply ignored. Unfortunately this results in designs that can be easily compromised by an adversary with realistic access to the {\em entire} device (including the state in the ignored layers). 

\begin{mybox}{}
Implementing PD in any one layer does not provide overall PD for the entire system
\end{mybox}

To see that, consider a typical PD scheme composed of two consecutive steps:

\begin{enumerate}

\item
\label[Step]{item:PD-step_1}
the scheme processes the input access request, and then outputs a sequence of operations that are meant to be executed on the underlying physical device (``{\em operation traces}'').

\item
\label[Step]{item:PD-step_2}
the operations traces are performed on the device.
\end{enumerate}

The typical adversary only gets to see snapshots of the physical device, and notably not the operations traces in \Cref{item:PD-step_1}. The scheme may be compromised if the traces get (even partially) leaked to the adversary, or modified before actual execution in \Cref{item:PD-step_2}.  

% Consider the scenario where SSDs are used as the underlying device for a \BD-layer PD scheme. At the first glance, this seems to be a reasonable combination. Indeed, SSDs are widely-known as a block device (aka \BD-layer device), which seems suitable for a \BD-layer PD scheme. However, this is actually a bad practice for the following reasons. 
A simple example where such compromise can easily occur is in flash. SSDs implement an \FTL layer inside-the-box that ``sees'' all operation traces before they are executed on the actual flash cells. However, the complex wear-leveling logic inside the \FTL maintains significant amount of state both in as meta information and on the device itself (un-mapped not-yet-ERASEd blocks containing compromising old data etc) that, when inspected can directly reveal critical information about past traces or even the traces themselves.

In general, {\bf a realistic adversary with visibility into the state of one or more other layers, can immediately compromise single-layer designs since that state can reveal access patterns and other security-sensitive information that a single-layer model simply cannot consider.}

PD designers should always state explicitly the requirements on the underlying devices with which their schemes are supposed to work; And engineers need to always check carefully that all such requirements are satisfied when implementing PD schemes.

\subsection{Removing Layer Dependency}
\label{sec:trace-oriented_PD}

The discussion in \Cref{sec:layer-dependency} leads to the following question:

\begin{itemize}
    \item[]{\em Is it possible to achieve a stronger PD whose security is independent of individual technology stack layers?}
\end{itemize}

The answer is yes. This section will discuss how. We note that layer-independence is preferable. First, it enables modularity and ensures end-to-end security. Second, it enables the evaluation of different schemes based on overall security strength. Performance metrics (e.g. time/space efficiency) also make better sense when they are least interwoven with stack layers. Otherwise, it is difficult to compare PD solutions operating on two different layers. Third, the fewer dependencies on implementation specifics, the better the security abstraction. PD can now be compared with other security constructs such as ORAMs; Such a connection is hard to establish for layer-dependent PD.  

The remainder of this section will first formalize a new layer-independent ``{\em trace-oriented}'' PD paradigm, and then investigate its security and efficiency implications. Importantly, it will be shown that {\em trace-oriented PDs are essentially equivalent to write-only ORAMs}.

\para{Defining Trace-Oriented PD}.
% \chen{Similarly, no game is given until now. All the analysis here should be moved to a section 6, which is after the unified game is proposed in section 5. Here, the only point that should be made clear is that there is a new kind of security -- trace-oriented security -- that could help getting rid of the constrains about storage levels. And there are already schemes that ensure trace-oriented security.}
In the security game of (standard) PD, the adversary sends challenge access requests and receives back snapshots of the physical device, resulted from the execution of the PD logic. Trace-oriented PDs are defined by modifying this security game in the following way: instead of the snapshots, the adversary will receive the operation traces (defined in \Cref{item:PD-step_1}) as the reply to its challenge requests in the security game. Namely, it is stipulated that the adversary cannot tell which of the two challenge sequences were executed, even if it gets to learn the outputs of the PD logic (aka operation traces), before they are physically executed on the storage medium. Intuitively, this is a stronger requirement than that of standard PD because operation traces may contain more information than snapshots---it is totally possible that two different sequences of operation traces lead to the same snapshot.

Moreover, note that the operations contained in the operation traces are either \texttt{Read} or \texttt{Write} operations. Only \texttt{Write} operations would potentially leave traces on the (snapshot of) storage medium. As argued in \Cref{remark:Read_for_free}, \texttt{Write} is the only type of operations that the trace-oriented definition needs to consider. Namely, it only requires that the \texttt{Write} traces reveals no information of the access requests to a PD scheme. Technically, consider a function $\mathsf{WOnly}(\cdot)$ which filters out the \texttt{Read} operations but passes the \texttt{Write} operations; The above security game is then modified by returning to the adversary the result of applying $\mathsf{WOnly}(\cdot)$ on operation traces. This constitutes the final definition of trace-oriented PDs.

\begin{remark}[On $\mathtt{Read}$ operations.]
\label{remark:Read_for_free}
The above choice to exclude $\mathtt{Read}$ operations is because that it is an unnecessary requirement that could incur inherent performance constraints. Jumping ahead, an analogue of \Cref{lemma:tPD_wORAM} will show that: including $\mathtt{Read}$ will lead to a trace-oriented PD definition that is equivalent to ORAMs (instead of write-only ORAMs), thus suffering ORAMs' efficiency lower-bounds \cite{goldreich1996software,boyle2016there,larsen2018yes,weiss2018there,hubavcek2019stronger}.
\end{remark}

It is not hard to see that a PD scheme meeting the trace-oriented definition also satisfies the standard PD definition. Indeed, \Write traces (the output of $\mathsf{WOnly}$) contain all the information to induce storage medium snapshots; If they are oblivious of the input access request, so are the snapshots. Furthermore, it resolves the issue of layer dependency: %in \Cref{sec:layer-dependecy}:
indistinguishable operation traces remain indistinguishable after being processed by arbitrary (polynomial-time) procedures. Therefore, \Lay-layer trace-oriented PD schemes allow the existence of extra layers between the PD logic and the physical devices. In particular, SSDs can be used if the \BD-layer PD scheme achieves trace-oriented security.

\begin{mybox}{}
Trace-oriented PD implies the standard PD security. Properly implemented trace-oriented PD secure mechanisms can provide PD for the entire system.
\end{mybox}

\para{Trace-Oriented PD in Practice.} In spite of all its advantages, this notion is useful only if it is also practical. Fortunately, the PD schemes  in \cite{blass2014toward,chakraborti2017datalair,chen2019} already achieved the trace-oriented security defined above. 

\chen{This summary is wrong. not all the traced-secure PD are based on write-only ORAMS. E.g: PD-DM is trace-oriented secure, but it is not based on ORAMs. Thanks to the freedom of use public accesses to hide hidden accesses in PD, PD-DM allow different P1 for different hidden access, which will makes it weak than ORAM. I think the conclusion we made is that trace-oriented secure PD can generate a ORAM only if P1 and P2 are independent from P\_hid in the term of content(the length can be related). So this part and the following part should be changed.}
\xiao{simply remove \cite{chen2019} from the above citations.}
\chen{I do not think removing one citation works. The problem is that the summarized point is wrong. Write-only ORAM = PD only when the PD has specific restrictions on adversaries in the game. I will change both the argument below and the prove.}

\para{Equivalence between Trace-Oriented PDs and Write-Only ORAMs.} 
Blass et al. \cite{blass2014toward} constructed a trace-Oriented PD scheme from $\wORAM$. Further, $\wORAM$ can also be constructed from trace-oriented PDs  (shown formally in \Cref{sec:wORAM_from_PDs}). This implies the following lemma:

%\begin{mybox}{}
\begin{lemma}\label{lemma:eq:woram-tpd}
Write-only ORAMs are both {\em sufficient and necessary} for trace-oriented PDs.
\end{lemma}
%\end{mybox} 

%\Cref{lemma:eq:woram-tpd} gives a full characterization of trace-oriented PD by establishing its equivalence to $\wORAM$s. Future progress on \wORAM lower-bounds will apply immediately to trace-oriented PDs. Established lower-bounds for ORAMs can be viewed as a signal of the inefficiency of $\wORAM$s, which translates into clues to the inefficiency of robust PD:
%
%\begin{mybox}{}
%Strongly-secure PD solutions feature inherent fundamental efficiency limits. Achieving efficient PD requires layer-dependency.
%\end{mybox}
%
%However, importantly, there is no {\em established} lower-bound for $\wORAM$s yet. Thus, the optimistic interpretation of \Cref{lemma:eq:woram-tpd} encourages us to seek efficient trace-oriented PDs. Given that all exiting trace-oriented PD solutions are built on top of $\wORAM$s, it will be interesting to have constructions that do not make {\em explicit} use of $\wORAM$s. Such constructions may circumvent the ORAM lower-bound (if it turns out it applies to $\wORAM$s). 


==> multi_vs_single.tex <==
%!TEX root=main.tex

\section{Threat Model. Security Goals}
\label{section:single-vs-multi}
This section will first provide the problem setup for PD, and then investigate the two flavors of PD: single-snapshot security and multi-snapshot security.
% Importantly, we try to reveal the obstacle of designing efficient multi-snapshot PD schemes, which is one of the main issues this work strives to address.


\para{Problem Setup.} Plausibly deniable storage systems allow users to store
public data (which do not require protection, and  are potentially known by the adversary), {\em and} sensitive hidden data (which needs to be protected). Such systems seek to protect against coercive adversaries who can compel the user to hand over secrete information (e.g.\ encryption keys). Under duress, the user may need to provide some information (e.g.\ keys to public data) that dismisses the adversary's suspicions, while most importantly denying the existence of the hidden data. 

It is worth noting that typically, PD systems only intend to hide the existence of hidden data, not the fact that ``the system in use is PD''. In fact, designing PD systems that e.g., look indistinguishable from regular storage -- i.e., in an attempt to hide their very use -- is an important direction for future research (see also \Cref{sec:future-direction}). Detailed PD adversarial model formalisms and definitions are in  \Cref{append-section:model}.
% , where we also review the CPA-game-based definition for PD in \cite{blass2014toward,chakraborti2017datalair}.  


\iffalse
    \para{Problem Setup.} Plausible deniability systems categorize data into multiple security levels. The data in a particular security level is revealed only on the provision of a level-specific secret e.g., a password, a decryption key etc. On startup, the system prompts the user for a secret; if the secret provided matches an existing entry, then the data in the corresponding security level and all lower security levels are revealed to the user. The system does not leak any information about the data in the higher security levels. The goal of plausible deniability systems is to ultimately hide the total number of security levels from an adversary that can coerce the user to hand over secrets for one (or more) security levels. Due to space constraint, we discuss the assumptions on the adversaries in \Cref{append-section:model}, where we also review the CPA-game-based definition for PD in \cite{blass2014toward,chakraborti2017datalair}.  
\fi

% \gray{[Another version of 
% Section II-A]

%     In this section, we first recall the threat model for PD, which formalizes the setup for this paper. Then we investigate the two flavors of PD: single-snapshot security and multi-snapshot security. Importantly, we try to reveal the obstacle of designing efficient multi-snapshot PD schemes,  which is one of the main issues this work strives to address.
    
%     \subsection{The Game-Based Definition for PD}
    
%     As mentioned earlier, the formal definition of PD already appeared in \cite{blass2014toward,chakraborti2017datalair}. Jumping ahead, we also present our unified definition that is closely related to the ones in \cite{blass2014toward,chakraborti2017datalair}. Therefore, to avoid repetition, in this part we only provide minimum formalism that is enough for the reader to get familiar with the setup and understand the remainder of this paper. 
    
%     \para{Notations.} We use $\SecPar$ for the security parameter. For a set $\mathsf{S}$ we use $x \pick \mathsf{S}$ to mean $x$ is sampled uniformly from $\mathsf{S}$. $\PPT$ denotes probabilistic polynomial time, $\poly(\cdot)$ denotes any polynomial function and $\negl(\cdot)$ denotes negligible function.
    
%     \para{Requests and Access Patterns.} A logical request is the unit of input in a $\sysname$ scheme. A request can be represented as $r = (\data, \addr, \op, \level)$), where $\data$ denotes the data value, $\op \in \Set{\Read, \Write}$ indicates the type of the request, $\addr$ denotes the address, and $\level \in \Set{\pub,\hid}$ indicates whether the data $\data$ should be protected ($\level = \hid$) from coercive adversaries or not ($\level = \pub$). An {\em access pattern} $\Pat$ is an ordered sequence of requests. Given two patterns $\Pat^0 = (r_1^0, \cdots, r_n^0)$ and $\Pat^1= (r_1^1, \cdots, r_m^1)$, we define the union of them as 
%     $$\Pat^0 \cup \Pat^1 \coloneqq (r_1^0, \cdots, r_n^0, r_1^1, \cdots, r_m^1).$$
    
%     \para{Modeling the System.}
%     The system initializes with security levels: {\em public level} and {\em hidden level}, with their own key $\Key_\pub$ and $\Key_\hid$ respectively. As revealed by their name, they are supposed to be used to handle public/hidden requests. A request to the system contains two clearly marked parts: operations $\Pat_\pub$ on public data and operations $\Pat_\hid$ on hidden data. Once a new request comes, it update the current state based on the request, the current state and the keys $(\Key_\pub,\Key_\hid)$. We require correctness as in any storage system. Jumping ahead, we also hope to make sure that users without $\Key_\pub$ (resp. $\Key_\hid$) can learn nothing about the public (resp. hidden) data, though she can still make request consists of both public and hidden parts.
    
%     \para{The Security Game for PD.}
%     Generally speaking, \sysname schemes plausibly deny the existence of hidden data by claiming that the state of storage devices are resulted from only public data. This requires that for a hidden operation, there should exist certain public operations such that the resulting device states are indistinguishable.  
%     Towards a more rigorous treatment, we formalize the security of \sysname schemes via a cryptographic game. This game is played between a coercive adversary $\Adv$ and a challenger $\Challenger$ running a \sysname scheme $\Sigma$. Intuitively, the challenger $\Challenger$ aims at hiding the existence of hidden requests by claiming that only public requests happened, while the adversary $\Adv$ aims at guessing whether any hidden request has been executed in the system by observing the state of storage device. 
    
%     At the beginning of the game, the public key $\Key_\pub$ is handed over to the coercive adversary $\Adv$ while a hidden key  $\Key_\hid$ is remain unrevealed. The $\Challenger$ picks a random bit $b \pick \bits$. 
%     \begin{itemize}
%     \item
%     \underline{Single-snapshot security.} The $\Adv$ is allows to interact with $\Challenger$ for polynomially many round. In each round, $\Adv$ issues tow access patterns $\Pat^0$ and $\Pat^1$ that share the same access requests to public data, but may contain different access requests to the hidden data. The $\Challenger$ will always execute $\Pat^b$. At the end of these interactions, $\Adv$ gets the snapshot of the physical device. $\Adv$ wins if it can guess the value $b$ correctly. The scheme $\Sigma$ is said to achieve single-snapshot PD if the winning probability of $\Adv$ is $\le \frac{1}{2} + \negl(\SecPar)$ (The term $\frac{1}{2}$ reflects the fact that the $\Adv$ can guess randomly and win the game with probability $\frac{1}{2}$).
%     \item
%     \underline{Multi-snapshot security.} This notion of security is defined identical to the single-snapshot one, only with the following exception. At the end of each of the polynomially-many round, the $\Adv$ get the snapshots of the underlying device. 
%     \end{itemize}
%     As aforementioned, we omit on purpose some details in the above formalism. For a thorough description, we refer the reader to \cite{chakraborti2017datalair} and \Cref{sec:device-def-detail}.
% }


\iffalse
    \subsection{Threat Model}
    \label{sec:adv}
    In a typical setting, a user's stored sensitive {\em hidden data} needs to be protected from powerful adversaries. A user may also possess less sensitive {\em public data} which does not require any special protection. Adversaries are coercive and can compel the user to hand over encryption keys. Further, the adversaries may also be able to take snapshots of the user's storage device. 
    % Under duress, the user may need to reveal keys to public data while denying the existence of the hidden data. 
    % this is not a threat model -- you are explaining how you are solving the problem
    %An effective PD system should therefore not only hide the contents of the hidden data but also its very existence.
    
    % As for observing storage devices, the coercive adversary is competent to check the hardware storage medium at the level of bits and gates. The action for an adversary to examine the hardware storage device once is called taking a ``snapshot'' of the device.
    
    \para{Modeling the System.}
    \todo{are you discussing the adversary here or telling us how you implement the system?!? not sure this should be here}
    A PD system stores both public data and hidden data on one storage device, and the public data and hidden data are encrypted with different encryption keys,  $K_{pub}$ and $K_{hid}$ respectively. (The keys may be securely derived from user-generated passwords or other more secure mechanisms.)
    The system can be used either in a public-only mode -- in which case the user can only access public data -- or in a public+hidden mode where the user can access both hidden and public data. 
    % To determine the mode of operation, the user provides appropriate passwords/keys (at boot time or when the device is plugged in after a reboot etc).
    For the public-only mode, the user needs to provide $K_{pub}$; to access also hidden data both $k_{hid}$ and $K_{pub}$ are required. 
    
    \para{Adversary.}
    % In addition, a coercive adversary is also competent to understand the design detail of \sysname mechanisms.
    % Yet it is worth noting that the coercive adversary is not allowed to observe the running state (caches etc.) of a storage system
    % or inject malicious codes into the system
    % . This is why a small amount of protected memory can be used in some of the existing schemes. 
    % However, it is required that the protected memory should be used at run time only rather than  consistently existing along the lifetime of storage devices. Otherwise, we assert that the security is weakened.
    % %Apart from the above common assumptions, there are different assumptions about the adversary in specific work, which will be introduced later in detail.  
    %
    In summary commonly-considered adversaries: 
    \todo{are we discussing what we think an adversary can do or what others have thought in the past? some of the assumptions below may not hold in certain scenarios -- maybe we should rewrite this a bit more towards discussing what other have thought and what the drawback and benefits of each assumption are}
    \begin{itemize}
    	\item are computationally bounded.
    	\item are capable of requesting encryption keys from users.
    	\item are rational -- i.e., they stop asking for additional encryption keys whenever he/she cannot prove the existence of any unrevealed data. 
    	\item are aware of the underlying design of the PD mechanism (no ``security by obscurity'')
    	\item are able to take snapshots of the storage device. 
    	\item cannot observe runtime system state (memory, caches etc.)
    	\item do not know whether multiple keys are used
    	\item cannot perform malicious code injection on the system used by the user
    \end{itemize}
    
    Many of these assumptions make sense in reality and some may not apply in certain scenarios. For example if a border guard is assumed to have enough access to take a laptop disk snapshot it may not be unreasonable to assume that the same border guard may also be able to install malicious code onto the same laptop. 
    
    In general however, adversaries are conditioned by situational constraints. In such cases, {\em adaptive PD schemes} can be designed to trade off adversarial power assumptions for increased performance/efficiency of the PD system. 
    
    %Some examples will be discussed later.
    
    % {\bf Firstly}, for example, an adaptive scheme could consider a limit on the viable number of storage device snapshots a coercive adversary is realistically able to take. 
     
    % At one extreme, coercive adversaries able to take merely one snapshot are called {\it single-snapshot}. For more than one snapshot, at different times they are called  {\it multi-snapshot}. 
    % For example, a nation state adversary capable of requesting physical accesses to a storage device anytime, is a multi-snapshot adversary. 
    % Obviously, multi-snapshot adversaries are more powerful than single-snapshot ones. Moreover, 
    % multi-snapshot adversaries occur more often in reality. Crossing a border twice, checking in airline luggage, living under an oppressive government with physical access to devices, leaving devices in untrusted places subject to ``hotel maid'' attacks, all these are instances of multi-snapshot opportunities for an adversary. 
    
    % Naturally, the security of a \sysname scheme should not break down completely (under reasonable user behavior) and should be resilient to such realistic externalities (hotel maids, border guards, airline checked luggage etc).
\fi


\iffalse
\chen{It is not correct to used game-based PD to summarize the threat model of PD as only 3 of existing work are based on game-based PD. For all the other work, they are not related to game based PD and their threat model is not defined with games. We need a generic description of the threat model to explain what is the PD problem.}
\subsection{The Game-Based Definition for PD}
\label{sec:Pd-game}
As mentioned earlier, the formal definition of PD already appeared in \cite{blass2014toward,chakraborti2017datalair}. Jumping ahead, we also present our unified definition that is closely related to the ones in \cite{blass2014toward,chakraborti2017datalair}. Therefore, to avoid repetition, in this part we only provide minimum formalism that is enough for the reader to get familiar with the setup and understand the remainder of this paper. 

\para{Notations.} We use $\SecPar$ for the security parameter. For a set $\mathsf{S}$ we use $x \pick \mathsf{S}$ to mean $x$ is sampled uniformly from $\mathsf{S}$. $\PPT$ denotes probabilistic polynomial time, $\poly(\cdot)$ denotes any polynomial function and $\negl(\cdot)$ denotes negligible function.

\para{Requests and Access Patterns.} A logical request is the unit of input in a $\sysname$ scheme. A request can be represented as $r = (\data, \addr, \op, \level)$), where $\data$ denotes the data value, $\op \in \Set{\Read, \Write}$ indicates the type of the request, $\addr$ denotes the address, and $\level \in \Set{\pub,\hid}$ indicates whether the data $\data$ should be protected ($\level = \hid$) from coercive adversaries or not ($\level = \pub$). An {\em access pattern} $\Pat$ is an ordered sequence of requests. Given two patterns $\Pat^0 = (r_1^0, \cdots, r_n^0)$ and $\Pat^1= (r_1^1, \cdots, r_m^1)$, we define the union of them as 
$$\Pat^0 \cup \Pat^1 \coloneqq (r_1^0, \cdots, r_n^0, r_1^1, \cdots, r_m^1).$$

\para{Modeling the System.}
The system initializes with security levels: {\em public level} and {\em hidden level}, with their own key $\Key_\pub$ and $\Key_\hid$ respectively. As revealed by their name, they are supposed to be used to handle public/hidden requests. A request to the system contains two clearly marked parts: operations $\Pat_\pub$ on public data and operations $\Pat_\hid$ on hidden data. Once a new request comes, it update the current state based on the request, the current state and the keys $(\Key_\pub,\Key_\hid)$. We require correctness as in any storage system. Jumping ahead, we also hope to make sure that users without $\Key_\pub$ (resp. $\Key_\hid$) can learn nothing about the public (resp. hidden) data, though she can still make request consists of both public and hidden parts.

\para{The Security Game for PD.}
Generally speaking, \sysname schemes plausibly deny the existence of hidden data by claiming that the state of storage devices are resulted from only public data. This requires that for a hidden operation, there should exist certain public operations such that the resulting device states are indistinguishable.  
Towards a more rigorous treatment, we formalize the security of \sysname schemes via a cryptographic game. This game is played between a coercive adversary $\Adv$ and a challenger $\Challenger$ running a \sysname scheme $\Sigma$. Intuitively, the challenger $\Challenger$ aims at hiding the existence of hidden requests by claiming that only public requests happened, while the adversary $\Adv$ aims at guessing whether any hidden request has been executed in the system by observing the state of storage device. 

At the beginning of the game, the public key $\Key_\pub$ is handed over to the coercive adversary $\Adv$ while a hidden key  $\Key_\hid$ is remain unrevealed. The $\Challenger$ picks a random bit $b \pick \bits$. 
\begin{itemize}
\item
\underline{Single-snapshot security.} The $\Adv$ is allows to interact with $\Challenger$ for polynomially many round. In each round, $\Adv$ issues tow access patterns $\Pat^0$ and $\Pat^1$ that share the same access requests to public data, but may contain different access requests to the hidden data. The $\Challenger$ will always execute $\Pat^b$. At the end of these interactions, $\Adv$ gets the snapshot of the physical device. $\Adv$ wins if it can guess the value $b$ correctly. The scheme $\Sigma$ is said to achieve single-snapshot PD if the winning probability of $\Adv$ is $\le \frac{1}{2} + \negl(\SecPar)$ (The term $\frac{1}{2}$ reflects the fact that the $\Adv$ can guess randomly and win the game with probability $\frac{1}{2}$).
\item
\underline{Multi-snapshot security.} This notion of security is defined identical to the single-snapshot one, only with the following exception. At the end of each of the polynomially-many round, the $\Adv$ get the snapshots of the underlying device. 
\end{itemize}
As aforementioned, we omit on purpose some details in the above formalism. For a thorough description, we refer the reader to \cite{chakraborti2017datalair} and \Cref{sec:device-def-detail}.
\fi
 
\para{Single-Snapshot Adversary.} Single-snapshot adversaries can see the device only once before eventually confronting the user and demanding access to information. 
% This is the earliest formalism of PD. It is proposed to guarantee security for one-time use. In such settings, the coercive adversary is limited to check the device only once (thus a ``single-snapshot'' adversary). Such a restriction on the adversarial behaviors 
This makes the design of efficient PD schemes significantly easier---indeed, a single snapshot (i.e., of a randomized encrypted device) does not leak much (if any) information beyond its size. For PD then, it may be sufficient to hide the sensitive data ``encrypted''\footnote{The double quotation marks are due to the fact that although most schemes use standard encryption, there are some schemes (e.g.~\cite{anderson1998steganographic}) using primitives such as secret-sharing instead.}, e.g., indistinguishable from random ``free'' device areas.
%This can be further broken down to the following two requirements: (1) the encrypted hidden data are pseudo-random; (2) the location of the hidden data on the device is oblivious to the adversary.

%Requirement (1) is easy to achieve as standard encryption schemes (e.g.~AES) do yield pseudo-random ciphertexts. Thus, previous work mainly focuses on requirement (2). \xiao{elaborate on this???}

\iffalse
Existing work falls along two major directions. The first one is inspired by the classical concept of {\em steganography}, i.e.~embedding relatively small messages within large cover-texts, such as \red{sending a message to a spy by adding imperceptible echo at certain places in an audio recording \cite{petitcolas1999information}.} \cite{anderson1998steganographic} was the first work that deployed steganography to build PD file systems. It was further optimized by later work \cite{mcdonald1999stegfs,pang2003stegfs}. This approach usually suffers from space inefficiency, data loss, and high performance overheads. It is not suited for larger amounts of data. 

The second direction \cite{Truecrypt,skillen2013mobiflage,jia2017deftl} deploys the idea of ``hidden volumes'' (as opposed to ``public volumes'') embedded within the device (e.g., in the free space regions). If the free space region is always filled with random data and the hidden volumes are encrypted randomized, adversaries cannot tell if the blocks marked ``free'' in the main volume are actually free or containing encrypted data that is part of a hidden volume.
\fi

\para{Multi-Snapshot Adversary.} Unfortunately, the protection provided by single-snapshot PDs can be completely vitiated once the adversary has the ability to take multiple ``snapshots'' of the device at different time points \cite{Czeskis:2008:DED:1496671.1496678}. This is not only a theoretical concern but in fact represents a majority of real-world adversaries. Multiple border crossings, evil maid attacks and many others are simple examples of multi-snapshot opportunities for determined adversaries. It is worth noting that even less-traveled devices such as data center servers may face inspections by overreaching authorities empowered by rubberhose or ill-devised laws. For multi-snapshot PDs, it is exponentially more difficult to balance the security-efficiency trade-off. Exploring this will be one of the main themes of \Cref{section:hide-hidden-access,section:depedence-on-layers}.
% Here, we provide an initial intuition. 

\iffalse
Consider a simple scheme that divides a storage device into two parts: a public and a hidden part, encrypted with $\Key_p$ and $\Key_h$ respectively. All encryption in this work will be considered randomized with IND-CPA semantic security properties. When coerced, a user hands out $\Key_p$ and (implicitly) claims that the hidden part contains free or random data due to previous use etc. This simple scheme achieves single-snapshot security. The encrypted hidden data is indistinguishable from random and without $\Key_h$, the coercive authority cannot uncover the existence of hidden data. 

Yet, the scheme fails when faced with a multi-snapshot adversary. Two device snapshots between which the user alters hidden data will immediately reveal something is going on. After all, why did the random, free space change between snapshots?

And while it may be tempting to attribute such changes to some re-randomization/re-initialization of the unused space, this will not sound plausible when the public data did {\em not} change in between two snapshots. To avoid this, it seems a solution may be to have the storage logic deploy a new rule ensuring re-randomization on ``unused'' space; and such a rule must be consistent with users' access to the public part, etc. 

The above example highlights the key difference between single-snapshot security and multi-snapshot secure. It also reveals an essential requirement for multi-snapshot PD---hiding the access to the hidden data. Namely, it requires not only that the adversary is ignorant of the existence of hidden data, but also that even the manipulation to hidden data cannot raise the adversary's suspicion. Given this insight, it is not surprising to see (in \Cref{section:hide-hidden-access}) that progress in this area centers mainly around hiding access to hidden data.

\begin{mybox}{}
The essence of multi-snapshot resilient PD systems lies in hiding the accesses to hidden data.
\end{mybox}

As an overall summary for this section, we remark that PD is easier to achieve in the single-snapshot setting. There exist multiple implementations with good performance. Unfortunately for more realistic multi-snapshot adversaries efficient PD schemes are much harder to achieve. Thus, multi-snapshot PD schemes with real-world efficiency are an important topic to continue to make progress on. The remainder of this paper will focus primarily on the multi-snapshot adversary.
\fi

% \section{One the Security Goals}

% \red{Add a transition paragraph here...
% \begin{itemize}
% \item
% We argue why IND-CPA is a good secure goal to achieve. We remark that IND-CPA has been used as the de facto standard for PD. But, to the best of our knowledge, no previous papers have explicitly reasoned about the validity of this choice (?). 

% We provide the explanation by drawing analogy with encryptions. We also conceive other possible styles such as semantic security and IND-CCA security and compare IND-CPA with them.
% \item
% We provide insights behind the designing principles of single and multi-snapshot secure schemes
% \end{itemize}
% }

% \subsection{Why is IND-CPA security the proper goal of PD?}
%     The first step toward provably secure PD schemes is to have a good definition. The earliest cryptographic formalism of PD appeared in \cite{blass2014toward,chakraborti2017datalair}, where a security game was presented analogous to the one used to define chosen-plaintext-secure (IND-CPA) encryptions. This definition then prevails in all the sequential work as the golden standard for PD. However, none of them (including \cite{blass2014toward,chakraborti2017datalair}) has ever argued for the adoption of such a definition. Without enough validation, certain perspectives of it may appear perplexing, especially to practitioners who does not enjoy ample cryptography background. For example, how and to what extend dose this definition capture the requirement of PD? Is there a stronger or weaker-yet-adequate variants of it? etc.

%     In this subsection, we strive to give a thorough consideration regarding this definition. We hope the discussion can clarify any doubts on this IND-CPA-style game, fortify our confidence on it as THE proper definition, and help practitioners gain enough intuitions and insights to connect seamlessly these theoretical conditions to real-world attacks.

% \red{talk about the goal of PD, what we are going to hide from the adversary and how we want to hide it.}

% \red{say that we will consider the definitions analogous to the successful paradigm developed originally for encryption. 
% \begin{itemize}
% \item semantic security is too weak for PD
% \item
% IND-CPA is a little bit over-killing. But it hard to imagine weaker yet sufficient definition that is easy to work with. So we are happy to take this conservative approach. We should not worry too much about this situation, as the same situation happens also in the definition of IND-CPA encryption. 
% \item
% IND-CCA does not fit the framework of PD
% \end{itemize}
% Therefore, IND-CPA is arguable the most proper way to define PD.
% }

==> under_explored_and_future_directions.tex <==
%!TEX root=main.tex

\section{Future Directions}
\label{sec:future-direction}
\para{Traced-Oriented Security.} Most existing PD solutions exploit the possibility that different traces may result in the same snapshot, which allows users to interpret hidden operations as public ones. However, such an advantage is lost in the trace-oriented setting, as the adversary obtains {\em actual} traces. Thus, it is necessary to remove any clues of the user's operations from the traces. But this goal is hard to achieve without relying on {\wORAM}s. Currently, three constructions---MobiCeal, PD-DM and ECD---seem to achieve this. However:
    \begin{itemize}
        \item
        \underline{MobiCeal} (1) distribution of dummy accesses leaks information about hidden operations; (2) it also needs to resolve collisions of hidden cell in a {\em secure} way. Fixing these problems will essentially lead to a \wORAM style construction.
        \item
        \underline{PD-DM} achieves trace-based security but it may need to postpone the processing of hidden requests until the arrival of enough public ``cover'' operations.
        \item
        \underline{ECD} relies on periodic updates and the rate of updates determines the throughout of hidden operations. To ensure on-time processing of hidden requests, one may try to set a high update rate at the expense of bandwidth , which may in turn hurts I/O performance. Also, to avoid data loss, the scheme ends up with a low space utilization design (see the discussion in \Cref{section:canonical-forms}).
    \end{itemize}
    The above discussion yields the following insight:
    \begin{mybox}{}
    It is challenging to build schemes achieving both trace-based security and good efficiency. Instead of striving for trace-based PD, a more promising direction for practitioners may be to take the approach illustrated in \Cref{sec:fine-tuned-solution}, and design PDs directly for the ``right'' layer.%\todo{do we want this paragraph to be a mini lesson?}
    \end{mybox}
    
\para{Multi-Snapshot Security.}
As discussed in \Cref{section:single-vs-multi}, it is quite challenging to have PD schemes against multi-snapshot adversaries. Existing solutions are still too slow. It is important to explore this further. 
% ; so we are looking forward to more schemes with better efficiency. Moreover, we distilled 3 major approaches to obtain multi-snapshot security; it is interesting to see more approaches to address this issue. 

% Multi-snapshot adversaries learn the changes in the device across different time points. Modifications to hidden data must cause observable changes in snapshots, for which plausible explanations are required. Note that standard encryption does no suffice for this purpose, because it only hide the content of the data, but not the fact that they are accessed. This is the major difficulty that PD needs to overcome.    

% In addition to the above under-explored points, the following represents interesting future research directions in the PD area:

\para{Indistinguishability.} To equip the user with more credibility in face of coercive authorities, it is desirable to have PD schemes
that hide not only contents but also the evidence that a particular system is being used to hide
data. This can be done by, e.g., making the scheme look indistinguishable to a off-the-shelf storage system:
%A PD scheme that looks indistinguishable to a off-the-shelf storage system (e.g. EXT4) will equip the user with more credibility in face of coercive authorities. This property is denoted as ``compatibility''\todo{who denotes it as compatibility ?! we may have a compatible system that is not indistinguishable but still compatible ... }, and fits well with the original spirit of the concept of PD. 
%The following schemes represent the initial results in this direction: 
\begin{itemize}
    \item
    \underline{StegFS
    \cite{mcdonald2000steganographic}} 
    is indistinguishable to EXT2, except that it needs additionally to maintain a bitmap. It is interesting to make this scheme fully compatible by removing the bitmap, while not compromising the security.
    \item
    \underline{INFUSE}
    %\cite{chen2020infuse} 
    is indistinguishable to YAFFS \cite{yaffs}. But there currently are two obstacles that prevent it from being practical. First, it has a limited capacity for hidden data. If too much hidden data are stored, the distribution of cell voltages may become suspicious. Second, this scheme requires the firmware support which allows precise manipulation on flash cell voltages. But current NAND flash chips do not have the corresponding interface admitting such manipulations. Partial programming are used to achieve approximate result, which is not precise enough.
    \end{itemize}
   

\para{Artificial Patterns.} Existing PD schemes try to match hidden operations to public ones. This makes the hidden operation rather ``passive''. Namely, to perform a hidden operation, the system has to wait until the occurrence of the related public operation. It also restricts the types of allowed hidden operations.
An ``active'' approach is to let the system fake artificial patterns whenever the user wants to perform hidden operations. Plenty of methods from the statistical/machine learning literature have potential for this purpose. 
% The construction in \cite{zuck2017preserving} falls into this category.




==> unified_framework.tex <==
%!TEX root=main.tex
% \section{Comparing Existing Schemes}
% \label{sec:unified-def-mainbody}

% As discussed in \Cref{section:intro:challenges}, it is desirable to have a security framework that unifies various customized definitions of PD. This section aims to provide such a model, and to conduct comparisons of security and performance among existing schemes.

% \subsection{Unified Definition}
% \label{section:definition}

% The CPA-Game for PD from \cite{blass2014toward,chakraborti2017datalair} defined in \Cref{section:single-vs-multi} is deeply integrated with the underlying application. New solutions have to repurpose this game to define PD at different system layer with specific underlying devices. Further, several constructions restricted the adversary's power in exchange for better efficiency, making it unclear how they fit into this game definition.

% In this section we introduce a unified definition that (1) generalizes the CPA game \Cref{section:single-vs-multi}, thus inherits all its advantages, e.g.~secure against CPA-style coercion attacks, applicable for both multi-snapshot and single-snapshot settings; (2) it encompasses existing constructions and admits comparisons among them (shown in \Cref{section:comparison}); (3) it can be instantiated for both the traditional device-oriented security model and the trace-oriented one proposed in \Cref{sec:trace-oriented_PD}.

% We present the definition for a device-oriented setting with multi-snapshot adversaries. A parameter $\Lay$ (e.g., $\Lay$ can be $\FS$, $\BD$, $\FTL$ etc.) is used to restrict the discussion on the scenario where the adversary is attacking an \Lay-device. The security game captures the restrictions on the adversary's power by introducing an extra parameter $R$, which can be instantiated by the designer. This leads to a more unified point of view, as all PD schemes indeed share the same abstraction modulo the parameters $\Lay$ and $R$. Further, comparisons of security strength among different schemes become possible by investigating the restrictiveness of their respective $R$ parameters. 

% \para{Layer-Specific Notations.} An $\Lay$-device is the device that can be deployed at layer $\Lay$. Similarly, an $\Lay$-request is a legitimate access ($\Read$ or $\Write$) request to layer $\Lay$. An $\Lay$-pattern $\Pat$ is an ordered sequence of $\Lay$-requests. Let $\Pat_1 \cup \Pat_2$ denote the concatenation of requests in pattern $\Pat_1$ and $\Pat_2$. More details are provided \Cref{sec:device-def-detail}.


% \begin{definition}%[$\Lay$-layer device-oriented PD ($\LdPD$)]
% For a layer $\Lay$ %\in \Set{\mathsf{FS}, \mathsf{BD}, \mathsf{FTL}}$ 
% and an $\Lay$-device $\Dev$, an {\em $\Lay$-layer device-oriented PD} ($\LdPD$) scheme $\Sigma$ consists of the following two algorithms $(\Setup, \Oper)$:
% \begin{itemize}
%     \item {\bf $\Setup(\SecPar, \Dev)$}:
%     this function provides the initial setups. It takes as input the security parameter $\SecPar$ and an \Lay-device $\Dev$. It outputs the tuple $(\Dev_\init, \Key_\pub, \Key_\hid)$, where $\Dev_\init$ is the initialized device, $\Key_\pub$ is the key used to protect the public data and $\Key_\hid$ is the key used to protect the hidden data.    
%     \item {\bf $\Oper(\Key_\pub, \Key_\hid, \Dev_\state, \Pat)$}:
%     It takes as input an \Lay-pattern $\Pat$, the current state $\Dev_\state$, and the key-pair $(\Key_\pub, \Key_\hid)$. If $\Pat$ is not a valid $\Lay$-pattern, the algorithm outputs $\bot$ and halts; Otherwise, it generates a new state $\Dev'$ accordingly, and updates the current state to $\Dev_\state \coloneqq \Dev'$. It outputs the updated state $\Dev_\state$. Denote this procedure as:
%     \vspace{-5pt}$$\Dev_\state \leftarrow \Oper(\Key_\pub, \Key_\hid, \Dev_\state, \Pat).\vspace{-5pt}$$
%     It is worth noting that $\Oper$ is a {\em stateful algorithm}, i.e., it may maintain some {\em internal} state across consecutive invocations\footnote{This internal state should not be confused with the device state $\Dev_\state$ in the input to $\Oper$.}.
% \end{itemize} 
% \label{def:dpd}
% \end{definition}

% \para{Correctness.} Before discussing PD requirements, correctness needs to be defined. Yet, PD systems may be designed for different layers, needs and devices. It is not easy to have a single formalization that captures all scenarios. For example, while the \BD layer only needs to support $\mathtt{Write}$ and $\mathtt{Read}$, the APIs supported by the \FS layer vary between designs, leading to diverse correctness requirements. But note that, for a given application, it is typically easy to define the desired functionality. Therefore, we simply state that the system should correctly achieve the desired functionality, and leave the specification of correctness to designers.

% \para{Multi-Snapshot $\Lay$-Device PD.} With the model formally defined, the security for a PD scheme can be formalized  by the CPA-style game in \Cref{figure:MuldPD}. This game is played between a coercive adversary $\Adv$ and a challenger $\Challenger$ running a PD scheme $\Sigma$. $\Adv$ only knows  $\Key_\pub$ (for the public data that the scheme is not trying to hide), but not $\Key_\hid$\footnote{Otherwise, there is nothing to protect.}. At each round, $\Adv$ is allowed to send two patterns $\Pat_0$ and $\Pat_1$. $\Pat_0$ is the concatenation of two public parts $\Pat^1_\pub$ and $\Pat^2_\pub$, while $\Pat_1$ is the concatenation of  $\Pat^1_\pub$ and an arbitrary hidden request pattern $\Pat_\hid$ (up to some restrictions that will be discussed soon). The challenger will always execute $\Pat_b$ for a $b \in \Set{0,1}$ pre-fixed randomly, and send back the snapshot of the device. It is required that adversary should not be able to tell which pattern gets executed. This captures the exact requirement of PD---the execution of hidden requests $\Pat_\hid$ now can be interpreted as some other public requests $\Pat^2_\pub$. Indeed, $\Adv$ cannot tell the difference by investigating the snapshots.

% \subpara{The Adversary's Requests.}
% Note the requirements put on the adversary's request patterns. First, $\Pat_0$ and $\Pat_1$ must share the same $\Pat^1_\pub$, as otherwise $\Adv$ (with $\Key_\pub$) can always win the game by checking the public data in the received snapshot. For a similar reason, requirement \ref{Multi-dPD:item:empty-hidden-request} is also necessary.

% The most important difference between this security game and previous ones lies in requirement \ref{Multi-dPD:item:scheme-specific-requirement}. Ideally, a scheme should be secure against all PPT adversaries. However, this is usually not easy to achieve in practice. Instead, people proposed practical solutions and proved their security by making additional assumptions on the adversary. And these assumptions vary from schemes to schemes. Actually, all these assumptions can be viewed as requirements on the $\Pat^1_\pub$ and $\Pat^2_\pub$ part of the adversary's requests in the security game. Thus, the game in \Cref{figure:MuldPD} generalizes them as two parameters $R^1$ and $R^2$. As will be shown in \Cref{section:comparison}, by instantiating these two parameters properly, this game can capture the security requirements of all existing PD systems. Moreover, this approach provides a way to compare different PD solutions---schemes with less restrictive $R^1$ and $R^2$ are more preferable in terms of security.

% \begin{definition}[Multi-Snapshot \Lay-Device \PD]
% \label{definition:MuldPD}
% Fix a layer $\Lay$.
% % \in \Set{\mathsf{FS}, \mathsf{BD}, \mathsf{FTL}}$. 
% A \sysname $\Sigma = (\Setup, \Oper)$ is {\em multi-snapshot \Lay-device \PD} %($\Lay\text{-}\MuldPD$) 
% if for any \PPT adversary $\Adv$, the following holds:
% \vspace{-0.5em}\begin{equation}
%     \Pr\big[\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar) = 1\big] \le 1/2 + \negl(\SecPar)\vspace{-0.5em}
% \end{equation}
% where $\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar)$ is defined in \Cref{figure:MuldPD}. 
% \end{definition}

% \para{Single-Snapshot Security.} This definition can be modified to capture single-snapshot security by asking the challenger to send $\Adv$ a single snapshot, only after $\Adv$ is done will all its $\poly(\SecPar)$ many requests.

% \para{Trace-Oriented Security.} \Cref{definition:MuldPD} also extends naturally to capture the trace-oriented PD notion (\Cref{sec:trace-oriented_PD}). To do that, in \Cref{Multi-dPD:item:states} the challenger will reply $\Adv$ with operation traces, instead of the snapshots of the physical device. Moreover, as discussed in \Cref{sec:trace-oriented_PD}, the $\mathsf{WOnly}(\cdot)$ function needs to be applied to screen out the $\Read$ operations from the traces before they are sent to $\Adv$.

% \begin{figure}[!tb]
%     \begin{center}
% \begin{footnotesize}
%     \fbox{
%     \begin{minipage}{\columnwidth-10pt}
%     Denote this game as $\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar)$. It is parameterized by a security parameter $\SecPar$, an \LdPD scheme $\Sigma=(\Setup, \Oper)$, and an adversary $\Adv$.
%     \begin{description}
%         \item[Initialization:] 
%         The challenger $\Challenger$ executes the setup algorithm to get $(\Dev_\init, \Key_\pub, \Key_\hid) \leftarrow \Setup(1^\SecPar)$. $\Key_\pub$ is given to $\Adv$. The current state is set as $\Dev_\state \coloneqq \Dev_\init$.
%         \item[Challenge:] 
%          $\Challenger$ picks a  random bit $b \pick \Set{0,1}$, and then executes the following steps with $\Adv$ for $\poly(\SecPar)$ times:
%         \begin{enumerate}[leftmargin=*]
%             \item \label{Multi-dPD:item:patterns}
%             The adversary $\Adv$ sends to $\Challenger$ two $\Lay$-patterns:
%             \vspace{-5pt}$$\Pat_0 \coloneqq \Pat_\pub^1 \cup \Pat_\pub^2 \quad \text{and} \quad
%             \Pat_1 \coloneqq \Pat_\pub^1 \cup \Pat_\hid,\vspace{-5pt}
%             $$  
%             where $(\Pat_\pub^1, \Pat_\pub^2, \Pat_\hid)$ satisfies the following requirement:
%             \begin{enumerate}[label=(\alph*)]
%                 \item 
%                 $\Pat^1_\pub$ and $\Pat^2_\pub$ contain only public requests;
%                 \item
%                 $\Pat_\hid$ contains only hidden requests;
%                 \item \label{Multi-dPD:item:empty-hidden-request}
%                 $\Pat_\pub^2$ must be $\varnothing$ if $\Pat_\hid$ is $\varnothing$;
%                 \item \label{Multi-dPD:item:scheme-specific-requirement}
%                 $\Pat_\pub^1$ and $\Pat_\pub^2$ additionally satisfy some {\em scheme-specific} requirements $R^1$ and $R^2$ respectively;
%             \end{enumerate}
            
%             \item 
%             Based on the selected bit $b$, $\Challenger$ executes the request pattern $\Pat_b$ on the device and updates the current device state as: 
%           \vspace{-5pt}$$
%             \Dev_\state \leftarrow \Oper(\Key_\pub, \Key_\hid, \Dev_\state, \Pat_b).\vspace{-5pt}
%             $$
%             \item \label[Step]{Multi-dPD:item:states}
%             The challenger $\Challenger$ then sends the newest $\Dev_\state$ to $\Adv$.  
%         \end{enumerate}
        
%         \item[Output:] The adversary $\Adv$, with the knowledge of $\Key_\pub$ and $\poly(\SecPar)$ states $\Dev_\state$'s obtained from Step \ref{Multi-dPD:item:states} in the {\bf Challenge} phase, outputs a bit $b'$. The game terminates with the output defined as $\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar) \coloneqq (b == b')$.
%     \end{description}
%     \end{minipage}
%     }
%     \end{footnotesize}
%     \end{center}\vspace{-8pt}
%     \caption{Security game for multi-snapshot, $\Lay$-device PDS}
%     \label{figure:MuldPD}
% \end{figure}

% \subsection{Comparison}
% \label{section:comparison}

% \begin{table*}[!h]
% \begin{footnotesize}
%     \begin{tabular}{  l | c | C{28pt} | C{38pt} | c  | C{38pt} | C{1.2cm} | C{0.6cm} | C{25pt} | C{2cm} }
%     \hline
%     {\bf Schemes} & {\bf Year} & {\bf Snapshot} & {\bf Security Type} & {\bf Layer} & {\bf I/O Perf.} \scriptsize{($\Pub$/$\Hid$)} & {\bf Space Util.}  &  {\bf Data Loss} & {\bf Add'l. Space} & {\bf Device}\\
%     \hline
%     StegFS98 \cite{anderson1998steganographic}& 98 & Sin & device & FS &  - & $\approx$15\% & \cmark & \xmark & General\\
%     \hline
%     StegFS99 \cite{mcdonald1999stegfs}& 99 & Sin & device & FS &  0.86/0.06 & - &  \cmark & \xmark & General\\
%     \hline
%     StegFS03 \cite{pang2003stegfs}& 03 & Sin & device & FS &  0.06 & $>$80\% & \cmark & \xmark & General\\
%     \hline
%     TrueCrypt \cite{Truecrypt}& 04 & Sin & device & BD &  - & 100\% & \cmark & \xmark & General\\
%     \hline
%     MobiFlage \cite{skillen2013mobiflage}& 13 & Sin & device & BD & 0.95 & 100\% & \cmark &   \xmark & General\\
%     \hline
%     MobiPluto \cite{10.1145/2818000.2818046}& 15 & Sin & device & BD & - & 100\% & \cmark &   \xmark & General\\
%     \hline
%     DEFTL \cite{jia2017deftl}& 17 & Sin & device & FTL &  - & 100\% & \xmark & \xmark & NAND flash\\
%     \hline
%     DEFY \cite{DBLP:conf/ndss/PetersGP15}& 15 & Mul & device & FS & - & 100\% & \cmark &  \cmark & NAND flash\\
%     \hline
%     MobiCeal \cite{chang2018mobiceal}& 18 & Mul & device & BD &  0.78 & - & \cmark & \xmark & General\\
%     \hline
%     INFUSE \cite{chen2020infuse}& 20 & Mul & device & FS &  0.94/0.03 & $>$100\% & \cmark & \xmark & Certain NAND flash\\
%     \hline
%     PEARL\cite{chen2020pearl}& 21 & Mul & device & FTL &  0.6/0.15 & 80\% & \cmark & \xmark & NAND flash\\
%     \hline
%     HIVE\cite{blass2014toward}& 14 & Mul & trace & BD &  - & 50\% & \xmark & \xmark & General\\
%     \hline
%     HIVE-B\cite{blass2014toward}& 14 & Mul & trace & BD &  0.004 & 50\% & \xmark & \cmark & General\\
%     \hline
%     DataLair\cite{chakraborti2017datalair}& 17 & Mul & trace & BD & 0.19/0.01 & 50\% & \xmark &  \cmark & General\\
%     \hline
%     ECD \cite{zuck2017preserving}& 17 & Mul & trace & FTL &  * & 52.5\% & \cmark & \cmark & NAND flash\\
%     \hline
%     PD-DM\cite{chen2019} & 19 & Mul & trace & BD &  0.10/0.07 & $\approx$50\% & \xmark & \xmark & General\\
%     \hline
%     \end{tabular}
% \caption{Comparison of Existing PD Schemes} 
% \label{tab:hierarchy}
% \vspace{-0.5cm}
% \end{footnotesize}
% \end{table*}

% As discussed earlier, existing PD solutions were proposed under different assumptions and models, which made the comparison of their security strengths a tricky task. Also, these schemes vary a lot in many other aspects such as the performance overhead, the scope of application etc. But these aspects cannot be interpreted accurately without a clean classification of schemes' security---it does not make much sense to compare the efficiency of two PD solutions that provide non-comparable security guarantees. The unified definition in \Cref{section:definition} provides a framework for security comparison among existing solutions. Based on this framework, this section will analyze existing PD schemes from a variety of aspects (summarized in \Cref{tab:hierarchy}) so that people can have a comprehensive understanding of these schemes and choose whatever fits best their applications.

% \para{Security Metrics.} The security guarantee of PD schemes is related to the assumptions made on adversaries, which can be captured by the above unified definition. Specifically, the frequency of snapshot and the type of security (listed in \Cref{tab:hierarchy}) categorize the scheme in coarse granularity, and the constraints $\Rule_1$ and $\Rule_2$ are used to characterize the power of adversaries in a finer way. 

% Before presenting the constraints on each scheme, let us interpret the meaning of these constraints:

% \begin{enumerate}
% \item An ideal scheme should be secure against all PPT adversaries (corresponding to empty $\Rule_1$ and $\Rule_2$). But no existing solutions achieve this level of security. $\Rule_1$ and $\Rule_2$ can be viewed as specifying a subset of all PPT adversaries against which a PD scheme is secure. Thus, these constraints provide a criterion for security comparison: {\em the more constrictive, the fewer adversarial behaviors are ruled out, resulting in a more powerful adversary and a more secure scheme}. 

% \item 
% The constraints also define under which conditions hidden operations can be executed safely. For example, the $\Rule^1_{\scriptscriptstyle{\sf DEFTL}}$ and $\Rule^2_{\scriptscriptstyle{\sf DEFTL}}$ for DEFTL below essentially say that the hidden operations can be perform with {\em any} public operation, as long as an $\mathtt{Unmount}$ is performed (together with the trigger post-processing), before the device is handed over to the coercive adversary. The constraints for other schemes can also be interpreted similarly. Thus, {\em the less constrictive the constraints, the more flexibility a scheme has in performing hidden operations}.
% \end{enumerate}

% The following  interprets the security of existing schemes by specifying their corresponding constraints, and draw comparisons along the way.

% \subpara{StegFS 98, 99, 03.}
% %\cite{anderson1998steganographic,mcdonald1999stegfs,pang2003stegfs}.
% The series of StegFSes are following the same model and share the same constraints:
% \begin{itemize}
%     \item $R^1_{\scriptscriptstyle{\sf StegFS}}$: no restrictions ($\Pat^1_\pub$ can be any public pattern); 
%     \item $R^2_{\scriptscriptstyle{\sf StegFS}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \subpara{TrueCrypt, MobiFlage.}
% The corresponding constraints can be illustrated as follows:
% \begin{itemize}
%     \item $R^1_{\scriptscriptstyle{\sf Tc\&Mf}}$: no restrictions; 
%     \item $R^2_{\scriptscriptstyle{\sf Tc\&Mf}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \para{Highlight:} The above schemes achieve security only against single-snapshot adversaries. Although these schemes are designed in different storage layers (\FS vs \BD), they share the same restrictions on the adversaries' choice of patterns, thus achieving identical security guarantee.

% \subpara{DEFTL} has the following constraints:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf DEFTL}}$: the last operation in $\Pat_\pub^1$ must be \texttt{Unmount};
% 	\item $\Rule^2_{\scriptscriptstyle{\sf DEFTL}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \subpara{DEFY} offers PD conditioned on constraints:
% \begin{itemize}
%         \item $\Rule^1_{\scriptscriptstyle{\sf DEFY}}$: $\Pat_\pub^1$ should contain some public operations, and the last operation in $\Pat_\pub^1$ must be \texttt{Unmount};
%         \item $\Rule^2_{\scriptscriptstyle{\sf DEFY}}$: $\Pat_\pub^2$ should contain public accesses that generate enough deleted pages to cover accesses in $\Pat_\hid$.
% \end{itemize}
% In addition, DEFY assumes the existence of a special area on the device that is hidden from the adversary. This is a strong constraint that may not be satisfied in reality. Thus, the security provided by DEFY is considered weaker than any of the schemes that does not assume the existence of such a hidden area.

% \para{Highlight:} Both $\Rule^1_{\scriptscriptstyle{\sf DEFTL}}$ and $\Rule^1_{\scriptscriptstyle{\sf DEFY}}$ require an \Unmount operation. This corresponds to the so called ``on-event'' adversaries in HIVE, which means that the adversary can access the storage device only after certain event (e.g.~an \Unmount operation) happens. 

% Comparing the above constraints, it can be seen that DEFY puts more restrictions on  the adversary than DEFTL does. However, it cannot be said that the security level of DEFTL is stronger. Because DEFY is targeted at multi-snapshot adversaries while DEFTL protects against only single-snapshot adversaries.

% \subpara{HIVE-B} has the following constraints:
% \begin{itemize}
% \item 
%     $\Rule^1_{\scriptscriptstyle{\sf HIVEB}}:$ no restrictions;
% \item 
%     $\Rule^2_{\scriptscriptstyle{\sf HIVEB}}:$ $\Pat_\pub^2$ and $\Pat_\hid$ must be of equal length (i.e.~containing the same number of requests).
% \end{itemize}

% \subpara{PEARL} has the following constraints:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf PEARL}}$: the last operation in $\Pat_\pub^1$ must be \texttt{Unmount};
% 	\item $\Rule^2_{\scriptscriptstyle{\sf PEARL}}$: $\Pat_\pub^2$ should generate $k$ 1st invalid page where $k$ is the length of $\Pat_\hid$. A pattern that can generate one 1st invalid page could be: 1) one public \Write followed by a public $\mathtt{Delete}$ to the same page; 2) one public \Write which has a correspondingly public \Write in $\Pat_\pub^1$. 
% \end{itemize}

% \subpara{HIVE.} This is another PD scheme proposed in the same paper as HIVE-B. It provides the same security guarantee as HIVE-B, but with different constraints:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf HIVE}}$: $\Pat_\pub^1$ and $\Pat_\hid$ must be of equal length;
% 	\item $\Rule^2_{\scriptscriptstyle{\sf HIVE}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \subpara{DataLair} introduces a parameter $\phi$ in the constraints:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf DataLair}}$: $\Pat_\pub^1$ should contain as least $\phi \times k$ public \Write operations where $k$ if the length of $\Pat_\hid$ and $\phi$ is a pre-defined parameter;
% 	\item $\Rule^2_{\scriptscriptstyle{\sf DataLair}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \subpara{PD-DM} shares a similar security nature to DataLair, except that it uses a predicate $IsExecutable()$, instead of the parameter $\phi$, to capture the constraints for $\Pat_\pub^1$:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf PDDM}}$: $IsExecutable(\Pat_\pub^1 + \Pat_\hid)$ should be true;
% 	\item $\Rule^2_{\scriptscriptstyle{\sf PDDM}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \subpara{MobiCeal}	was originally proposed for mobile devices \bogdan{Radu: where does this solution fit, ORAM, canonical form, or device-specific mechanisms? I don't see it described anywhere. Maybe remove?} . But their technique can be generalized for other devices. Its constraints can be summarized as follows:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf MobiCeal}}$: $\Pat_\pub^1$ should contain some public operations so that the number of dummy writes generated together with those public operations plus the number of block writes resulting from $\Pat_\hid$ should be able to be claimed as dummy writes generated alone with the public operations in $\Pat_\pub^1$.
% 	\item $\Rule^2_{\scriptscriptstyle{\sf MobiCeal}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \subpara{ECD} has the following constraints:
% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf ECD}}$: no restrictions;
% 	\item $\Rule^2_{\scriptscriptstyle{\sf ECD}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}
% Note that ECD has the least restrictive rules compared with other schemes. This is because it employs a regular system behavior which periodically modifies the state of the device to cover up the hidden operation (details in \Cref{section:canonical-forms}); And such a periodic system update is general enough to cover any type of hidden operations. In contrast, other schemes use public operations to cover up hidden operations, which naturally introduces constraints to ensure that the public and hidden operations are ``paired'' properly.

% \para{Highlight:} HIVE, DataLair, PD-DM and MobiCeal provide multi-snapshot security at $\BD$ layer, with comparable constraints. Except for MobiCeal, all other schemes achieve the stronger trace-oriented security. Thus, by comparing their corresponding constraints, these schemes form the following security hierarchy:  HIVE $=$ DataLair $>$ PD-DM $>$ MobiCeal.

% \subpara{INFUSE} has the following constraints:

% \begin{itemize}
% 	\item $\Rule^1_{\scriptscriptstyle{\sf INFUSE}}$: the last operation in $\Pat_\pub^1$ must be \texttt{Unmount};
% 	\item $\Rule^2_{\scriptscriptstyle{\sf INFUSE}}$: $\Pat_\pub^2$ must be an empty pattern.
% \end{itemize}

% \para{Performance Metrics.} 
% \Cref{tab:hierarchy} also looks at existing solutions from a performance standpoint.

% \subpara{I/O Performance.} PD comes with both throughput and space overheads. Some schemes report performance separately for public operations and hidden operations -- shown in \Cref{tab:hierarchy} in the form of ``$x$/$y$''. It means that the public throughput is $x$ times of the non-PD baseline, and the hidden throughput is $y$ times of the baseline. Some other schemes reported only one overall performance number, and some schemes did not provide any explicit performance number or even have not been evaluated at all since they are designed in theory and no implementation is completed (shown as ``-'' in \Cref{tab:hierarchy}). 
% ECD is a special case whose performance (marked with ``*'' in the table) depends on a system parameter. Recall that ECD covers up hidden operations by periodically updating the device state at a prefixed rate $r$. Thus, the number of hidden operations that the system is able to performed is determined by the updating rate $r$, rather than the public operations happened.

% \subpara{Space Utilization.} The column ``{\bf Space Util.}'' shows how efficiently the storage capacity of physical devices can be exploited by each PD scheme. It is computed as the ratio {\em between} the max size of data (both public and hidden) that can be stored in one device {\em and} the total capacity of the storage device as a metric for space utilization in \Cref{tab:hierarchy} (space required by meta-data is excluded for simplicity). Note that INFUSE enjoys a space utilization larger than 100\%. That is because INFUSE encodes hidden bits at physical storage cells that already contains some public data (see \Cref{sec:fine-tuned-solution}).

% \subpara{Additional Safe Space, Data Loss.} As discussed in earlier sections, some PD solutions assume the existence of an area on the devices that remains hidden from adversaries (e.g.~the ``TSA'' block in DEFY, the stash in HIVE etc.). Some schemes suffer from data loss, i.e.~the hidden data may be overwritten (maybe by public data) in some use cases. \Cref{tab:hierarchy} also lists these caveats for each scheme.

% \begin{table*}[!ht]
% \begin{center}
% \begin{small}
%     \begin{tabular}{ | l | c | C{0.6cm} | C{32pt} | c  | C{38pt} | C{1.2cm} | C{0.6cm} | C{25pt} | C{1.2cm} |}
%     % \hline
%     % \multirow{3}{*}{Scheme(s)} & \multirow{3}{*}{Year} & \multirow{3}{*}{Snapshot} & \multirow{3}{*}{Type} & \multirow{3}{*}{Layer} & \multirow{3}{*}{Data Loss} & \multirow{3}{*}{Performance} & \multirow{3}{*}{Space Utilization} & \multirow{3}{*}{Security Level} & \multirow{3}{*}{Add'l. Safe Space} & \multirow{3}{*}{Device} \\
%     \hline
%     {\bf Schemes} & {\bf Year} & {\bf Snapshot} & {\bf Security Type} & {\bf Layer} & {\bf I/O Perf.} \scriptsize{($\Pub$/$\Hid$)} & {\bf Space Util.}  &  {\bf Data Loss} & {\bf Add'l. Safe Space} & {\bf Device}\\
%     \hline
%     % Scheme(s) & Year & Snap- & Type & Layer & Data & I/O & Space & Security & Add'l. & Device\\
%     % & & shot & & & loss & Perfor- & Utilization & level & Safe & \\
%     % & & & & & & mance & & & Space & \\
%     % \hline
%     StegFS98 \cite{anderson1998steganographic}& 98 & Sin & device & FS &  - & $\approx$15\% & \cmark & \xmark & General\\
%     \hline
%     StegFS99 \cite{mcdonald1999stegfs}& 99 & Sin & device & FS &  0.86/0.06 & - &  \cmark & \xmark & General\\
%     \hline
%     StegFS03 \cite{pang2003stegfs}& 03 & Sin & device & FS &  0.06 & $>$80\% & \cmark & \xmark & General\\
%     \hline
%     Truecrypt \cite{Truecrypt}& 04 & Sin & device & BD &  - & 100\% & \cmark & \xmark & General\\
%     \hline
%     Mobiflage \cite{skillen2013mobiflage}& 13 & Sin & device & BD & 0.95 & 100\% & \cmark &   \xmark & General\\
%     \hline
%     PEARL\cite{chen2020pearl}& 21 & Mul & device & FTL &  0.6/0.15 & 80\% & \cmark & \xmark & NAND flash\\
%     \hline
%     DEFTL \cite{jia2017deftl}& 17 & Sin & device & FTL &  - & 100\% & \xmark & \xmark & NAND flash\\
%     \hline
%     DEFY \cite{DBLP:conf/ndss/PetersGP15}& 15 & Mul & device & FS & - & 100\% & \cmark &  \cmark & NAND flash\\
%     \hline
%     INFUSE \cite{chen2020infuse}& 20 & Mul & device & FS &  0.94/0.03 & $>$100\% & \cmark & \xmark & Certain NAND flash\\
%     \hline
%     HIVE\cite{blass2014toward}& 14 & Mul & trace & BD &  - & 50\% & \xmark & \xmark & General\\
%     \hline
%     HIVE-B\cite{blass2014toward}& 14 & Mul & trace & BD &  0.004 & 50\% & \xmark & \cmark & General\\
%     \hline
%     DataLair\cite{chakraborti2017datalair}& 17 & Mul & trace & BD & 0.19/0.01 & 50\% & \xmark &  \cmark & General\\
%     \hline
%     PD-DM\cite{chen2019} & 19 & Mul & trace & BD &  0.10/0.07 & $\approx$50\% & \xmark & \xmark & General\\
%     \hline
%     MobiCeal \cite{chang2018mobiceal}& 18 & Mul & device & BD &  0.78 & - & \cmark & \xmark & General\\
%     \hline
%     ECD \cite{zuck2017preserving}& 17 & Mul & device & FTL &  * & $<$75\% & \xmark & \xmark & NAND flash\\
%     \hline
%     \end{tabular}
% \caption{Comparison of Existing PD Schemes (symbol ``-'' indicates that data is not explicitly reported in related paper).}
% \label{tab:hierarchy}
% \end{small}
% \end{center}
% \end{table*}


% Although different definitions for PD appeared in the literature, they fall short in several aspects: 
% \begin{itemize}
% \item
% these definitions are usually highly tailored to specific applications or constructions. For example, the security game used in \cite{blass2014toward} serves well for their \red{Hidden volume technique for Block-device layer}, but non-trivial modifications are needed to adapt this model to other constructions or discussing PDs at other storage layers; 
% \item
% there is a mismatch between these definitions and the practice of PD research.
% Following the convention of cryptography, these definitions require security against arbitrary probabilistic polynomial time (PPT) adversary. However, until today, all practical PD schemes fail to meet this requirement. This leads to two undesirable effects:
% \begin{itemize}
% \item since it is hard to conduct rigorous security proof according to such an ideal definition, several papers turned to showing heuristic evidence for security. This could be dangerous. For example, DEFY \cite{DBLP:conf/ndss/PetersGP15} was asserted to be secure based on the heuristic that a hidden page was indistinguishable from a secure-deleted public page. However, Jia et al.~\cite{jia2017deftl} later showed that DEFY could be compromised if adversaries makes several attempts to exhaust the writing capacity.
% \item
% for constructions that fail to meet such definitions (this includes all practical PD schemes unknown today), there is no good way to interpret/understand their security strength; this also makes it hard to draw comparisons among these practical constructions. 
% \end{itemize} 
% \end{itemize} 
% Therefore, it becomes urgent to have a unified definition that adapts well to the practice of PD research, and  captures the most essence of PD, being independent as much as possible of devices and application details.
% \begin{mybox}{}
% It is important to use a unified model that can properly compare security and performance trade-offs between different systems. 
% \end{mybox}


% \subsection{Our Unified Definition} 
% \label{sec:unified-def-mainbody}
% In this part, we present a unified definition for PD.
% It encompass existing definitions, and allows comparisons of performance among existing solutions. It also extends naturally to the trace-based security proposed in \Cref{sec:trace-oriented_PD}.

% Our starting point is the PD definitions in \cite{blass2014toward,chakraborti2017datalair}. Blass et al.~\cite{blass2014toward} was the first one to formalize PD using a CPA-style security game. But as mentioned earlier, that game was ad hoc to their hidden volume encryption format, and did not adapt to other constructions. Also, although their game assumed arbitrary PPT adversaries, the {\em practical} constructions proposed in  \cite{blass2014toward} were not strong enough to satisfy such a definition\footnote{We note that one of their constructions (based on $\wORAM$s) provably achieved this definition. But it is too inefficient to be practical.}. For those schemes, they only discussed heuristic evidences for security when different types of restrictions were put on adversaries' behavior. Based on the model in \cite{blass2014toward}, Chakrabort et al.~\cite{chakraborti2017datalair} proposed a conceptually cleaner CPA game for PD. Instead of allowing arbitrary PPT adversarial behaviors, it ``hardwires'' the restrictions (ad hoc to DataLair's construction) on the adversary's requests into the security game.


% We follow the CPA paradigm established by \cite{blass2014toward,chakraborti2017datalair} but with the following modification. We first use a parameter $\Lay \in \Set{\FS, \BD, \FTL}$ to restrict the discussion on the scenario where an \Lay adversary is attacking an \Lay-device. Then, we capture the restrictions on the adversarial requests (in the security game) by introducing an extra parameter $R$, which can be instantiated to designer's choice. This leads to a more unified point of view, as all PD schemes indeed share the same abstraction modulo the parameters $\Lay$ and $R$; and comparisons of security strength among different schemes become possible by investigating the restrictiveness of their respective $R$ parameters. 

% In the following, we first present the notations and syntax for PD scheme, and then present the formal security requirement in \Cref{definition:MuldPD}.

% \para{Layer-Specific Notations.} For $\Lay \in\Set{\FS, \BD, \FTL}$, an $\Lay$-device is the device that can be deployed at layer $\Lay$. Similarly, an $\Lay$-request is a legitimate access ($\Read$ or $\Write$) request to layer $\Lay$. An $\Lay$-pattern $\Pat$ is an ordered sequence of $\Lay$-requests. We use $\Pat_1 \cup \Pat_2$ to denote the concatenation of requests in pattern $\Pat_1$ and $\Pat_2$. For more details, see \Cref{sec:device-def-detail}.


% \begin{definition}%[$\Lay$-layer device-oriented PD ($\LdPD$)]
% Given an $\Lay \in \Set{\mathsf{FS}, \mathsf{BD}, \mathsf{FTL}}$ and an $\Lay$-device $\Dev$, an {\em $\Lay$-layer device-oriented PD} ($\LdPD$) scheme $\Sigma$ consists of the following two algorithms $(\Setup, \Oper)$:
% \begin{itemize}
%     \item {\bf $\Setup(\SecPar, \Dev)$}:
%     this function provides the initial setups. It takes as input the security parameter $\SecPar$ and an \Lay-device $\Dev$. It outputs the tuple $(\Dev_\init, \Key_\pub, \Key_\hid)$, where $\Dev_\init$ is the initialized device, $\Key_\pub$ is the key used to protect the public data and $\Key_\hid$ is the key used to protect the hidden data.    
%     \item {\bf $\Oper(\Key_\pub, \Key_\hid, \Dev_\state, \Pat)$}:
%     It takes as input an \Lay-pattern $\Pat$, the current state $\Dev_\state$, and the key-pair $(\Key_\pub, \Key_\hid)$. If $\Pat$ is not a valid $\Lay$-pattern, the algorithm outputs $\bot$ and halts; otherwise, it generates a new state $\Dev'$ accordingly, and updates the current state to $\Dev_\state \coloneqq \Dev'$. It outputs the updated state $\Dev_\state$. We refer to this procedure as:
%     $$\Dev_\state \leftarrow \Oper(\Key_\pub, \Key_\hid, \Dev_\state, \Pat).$$
%     We remark that $\Oper$ is a {\em stateful algorithm}, i.e. it may maintain some {\em internal} state across consecutive invocations\footnote{This internal state should not be confused with the device state $\Dev_\state$ in the input to $\Oper$.}.
%     %\item {\bf $\PostPro(\Key_\pub, \Key_\hid, \Dev_\state)$}:
%     %    this function describes the post-processing procedure in a scheme $\Sigma$. It is executed before the adversary's coercion happens.  It takes as input the current state $\Dev_\state$ and the key-pair $(\Key_\pub, \Key_\hid)$, and outputs the post-processed version device state $\overline{\Dev}_\state$. We refer to this process as    $$\overline{\Dev}_\state \leftarrow \PostPro(\Key_\pub, \Key_\hid, \Dev_\state).$$ Note that not all $\LdPD$ schemes have a post-processing. In other words, $\PostPro$ can be simply an identity function, i.e. $\overline{\Dev}_\state = \Dev_\state$.
% \end{itemize} 
% \label{def:dpd}
% \end{definition}

% \para{Multi-Snapshot $\Lay$-Device PDS.} With the model formally defined, we are now ready to formalize the security definition for PDS by the CPA-style game in \Cref{figure:MuldPD}. This game is played between a coercive adversary $\Adv$ and a challenger $\Challenger$ running a \sysname scheme $\Sigma$. We give $\Adv$ only $\Key_\pub$ (for the public data that we are not trying to hide), but not $\Key_\hid$\footnote{Otherwise, there is nothing to protect.}. At each round, $\Adv$ is allowed to send two patterns $\Pat_0$ and $\Pat_1$. $\Pat_0$ is the concatenation of two public parts $\Pat^1_\pub$ and $\Pat^2_\pub$, while $\Pat_1$ is the concatenation of  $\Pat^1_\pub$ and an arbitrary hidden request pattern $\Pat_\hid$ (up to some restrictions that we will discuss soon). The challenger will always execute $\Pat_b$ for a $b \in \Set{0,1}$ pre-fixed randomly, and send back the snapshot of the device. It is required that adversary should not be able to tell which pattern gets executed. This captures the exact requirement of PD---the execution of hidden requests $\Pat_\hid$ now can be interpreted as some other public requests $\Pat^2_\pub$; indeed, $\Adv$ cannot tell the difference by investigating the snapshots.




% \subpara{The Adversary's Requests.} We want to highlight the restrictions put on the adversary's request patterns. First, $\Pat_0$ and $\Pat_1$ share the same $\Pat^1_\pub$, as otherwise $\Adv$ (with $\Key_\pub$) can always win the game by checking the public data in the received snapshot. For a similar reason, requirement \ref{Multi-dPD:item:empty-hidden-request} is also necessary.

% The most important difference between our security game and previous ones lies in requirement \ref{Multi-dPD:item:scheme-specific-requirement}. Ideally, we want a scheme to be secure against all PPT adversaries. However, this is usually not easy to achieve in practice. Instead, people proposed practical solutions and proved their security by making additional assumptions on the adversary. And these assumptions vary from schemes to schemes. We observe that all these assumptions can be viewed as restrictions on the $\Pat^1_\pub$ and $\Pat^2_\pub$ part of the adversary's requests in the security game. Thus, we generalize them as two parameters $R^1$ and $R^2$. As we will show in \Cref{section:security-hierarchy}, by instantiating these two parameters properly, our game can capture the security requirements of all existing PD systems. Moreover, this approach provides a way to compare different PD solutions---schemes with less restrictive $R^1$ and $R^2$ are more preferable in terms of security.

% \begin{definition}[Multi-Snapshot \Lay-Device \PD]
% \label{definition:MuldPD}
% Fix a layer $\Lay \in \Set{\mathsf{FS}, \mathsf{BD}, \mathsf{FTL}}$. A \sysname $\Sigma = (\Setup, \Oper)$ is {\em multi-snapshot \Lay-device \PD} ($\Lay\text{-}\MuldPD$) if for any \PPT adversary $\Adv$, the following holds:
% \begin{equation}
%     \Pr\big[\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar) = 1\big] \le \frac{1}{2} + \negl(\SecPar)
% \end{equation}
% where $\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar)$ is defined in \Cref{figure:MuldPD}. 
% \end{definition}

% \para{Single-Snapshot Security.} Our definition can be modified to capture single-snapshot security by asking the challenger to send $\Adv$ a single snapshot, only after $\Adv$ is done will all its $\poly(\SecPar)$ many requests. We denote such security as $\Lay\text{-}\SindPD$. Due to space constrains, we omit the formal description of the single-snapshot security game.

% \para{Trace-Oriented Security.} Our definition also extends naturally to capture the trace-oriented PD notion (\Cref{sec:trace-oriented_PD}). To do that, in \Cref{Multi-dPD:item:states} the challenger will reply $\Adv$ with operation traces, instead of the snapshots of the physical device. Moreover, as discussed in \Cref{sec:trace-oriented_PD}, we need to apply the $\mathsf{WOnly}(\cdot)$ function to screen out the $\Read$ operations from the traces before they are sent to $\Adv$. We provide more details in \Cref{sec:trace-def-detail}. We denote the the single-snapshot and multi-snapshot trace-oriented PDS for layer $\Lay$ as $\Lay\text{-}\SintPD$ and $\Lay\text{-}\SintPD$ respectively.


% \begin{figure}[!htb]
%     \begin{center}
%     \fbox{
%     \begin{minipage}{\columnwidth-10pt}
%     We denote this game as $\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar)$. It is parameterized by a security parameter $\SecPar$, an \LdPD scheme $\Sigma=(\Setup, \Oper)$, and an adversary $\Adv$.
%     \begin{description}
%         \item[Initialization:] 
%         The challenger $\Challenger$ executes the setup algorithm to get $(\Dev_\init, \Key_\pub, \Key_\hid) \leftarrow \Setup(1^\SecPar)$. $\Key_\pub$ is given to $\Adv$. The current state is set as $\Dev_\state \coloneqq \Dev_\init$.
%         \item[Challenge:] 
%          $\Challenger$ picks a  random bit $b \pick \Set{0,1}$, and then executes the following steps with $\Adv$ for $\poly(\SecPar)$ times:
%         \begin{enumerate}[leftmargin=*]
%             \item \label{Multi-dPD:item:patterns}
%             The adversary $\Adv$ sends to $\Challenger$ two $\Lay$-patterns:
%             $$\Pat_0 \coloneqq \Pat_\pub^1 \cup \Pat_\pub^2 \quad \text{and} \quad
%             \Pat_1 \coloneqq \Pat_\pub^1 \cup \Pat_\hid,
%             $$  
%             where $(\Pat_\pub^1, \Pat_\pub^2, \Pat_\hid)$ satisfies the following requirement:
%             \begin{enumerate}[label=(\alph*)]
%                 \item 
%                 $\Pat^1_\pub$ and $\Pat^2_\pub$ contain only public requests;
%                 \item
%                 $\Pat_\hid$ contains only hidden requests;
%                 \item \label{Multi-dPD:item:empty-hidden-request}
%                 $\Pat_\pub^2$ must be $\varnothing$ if $\Pat_\hid$ is $\varnothing$;
%                 \item \label{Multi-dPD:item:scheme-specific-requirement}
%                 $\Pat_\pub^1$ and $\Pat_\pub^2$ additionally satisfy some {\em scheme-specific} requirements $R^1$ and $R^2$ respectively;
%             \end{enumerate}
            
%             \item 
%             Based on the selected bit $b$, $\Challenger$ executes the request pattern $\Pat_b$ on the device and updates the current device state as: 
%             $$
%             \Dev_\state \leftarrow \Oper(\Key_\pub, \Key_\hid, \Dev_\state, \Pat_b).
%             $$
%             \item \label[Step]{Multi-dPD:item:states}
%             %The challenger $\Challenger$ conducts post-processing on the current state by $$ \overline{\Dev}_\state \leftarrow \PostPro(\Key_\pub, \Key_\hid, \Dev_\state).$$ 
%             The challenger $\Challenger$ then sends the newest $\Dev_\state$ to $\Adv$.  
%         \end{enumerate}
        
%         \item[Output:] The adversary $\Adv$, with the knowledge of $\Key_\pub$ and $\poly(\SecPar)$ states $\Dev_\state$'s obtained from Step \ref{Multi-dPD:item:states} in the {\bf Challenge} phase, outputs a bit $b'$. The game terminates with the output defined as $\MuldPD^{\Lay}_{\Sigma,\Adv}(\SecPar) \coloneqq (b == b')$.
        
%     \end{description}
%     \end{minipage}
%     }
%     \end{center}
%     \caption{Security game for multi-snapshot, $\Lay$-device PDS}
%     \label{figure:MuldPD}
% \end{figure}


% \subsection{A Hierarchy Based on the Power of Adversaries}
% \label{section:security-hierarchy}
% \begin{table}[!h]
%     \begin{center}
%         \def\arraystretch{1}
%         \begin{tabular}{ |C{0.6cm} | L{0.5cm} | L{2.2cm} | L{2.5cm} |}
%         \hline
%         \multicolumn{2}{|c|}{} & Multi-Snapshot& Single-Snapshot \\
%             \hline
%             \multirow{3}{*}{Trace}  &  FS & -- & -- \\
%                                     \cline{2-4} 
%                                     &  BD & HIVE-B, HIVE, DataLair, PD-DM & -- \\
%                                     \cline{2-4} 
%                                     &  FTL & -- & -- \\
%             \hline
%             \multirow{3}{*}{Device} &  FS & DEFY, INFUSE & StegFS98, StegFS99, StegFS03 \\
%                                     \cline{2-4} 
%                                     &  BD & -- & Truecrypt, Mobiflage \\
%                                     \cline{2-4} 
%                                     &  FTL & PEARL & DEFTL \\
%             \hline
%         \end{tabular}
%         \caption{Comparison of Existing PD Schemes}
%         \label{tab:hierarchy}
%     \end{center}
% \end{table}

% In \Cref{tab:hierarchy}, we categorize existing PDS schemes according to our definitional framework from \Cref{sec:unified-def-mainbody}. Roughly, the tale is arrange in a way such that the security strength of the schemes decreases from top to bottom, left to right.

